Satire: Computing Rigorous Bounds for Floating-Point Rounding Error in Mixed-Precision Loop-Free Programs

Techniques that rigorously bound the overall rounding error exhibited by a numerical program are of significant interest for communities developing numerical software. However, there are few available tools today that can be used to rigorously bound errors in programs that employ conditional statements (a basic need) as well as mixed-precision arithmetic (a direction of significant future interest) employing global optimization in error analysis. In this paper, we present a new tool that fills this void while also employing an abstraction-guided optimization approach to allow designers to trade error-bound tightness for gains in analysis time -- useful when searching for design alternatives. We first present the basic rigorous analysis framework of Satire and then show how to extend it to incorporate abstractions, conditionals, and mixed-precision arithmetic. We begin by describing Satire's design and its performance on a collection of benchmark examples. We then describe these aspects of Satire: (1) how the error-bound and tool execution time vary with the abstraction level; (2) the additional machinery to handle conditional expression branches, including defining the concepts of instability jumps and instability window widths and measuring these quantities; and (3) how the error changes when a mix of precision values are used. To showcase how \satire can add value during design, we start with a Conjugate Gradient solver and demonstrate how its step size and search direction are affected by different precision settings. Satire is freely available for evaluation, and can be used during the design of numerical routines to effect design tradeoffs guided by rigorous empirical error guarantees.

==> Abstractions/files/abstraction_heuristic.tex <==
\subsection{An Information-theoretic Abstraction Heuristic}

We now introduce a practical and automated abstraction heuristic that integrates a combination of competing factors to achieve scalability and precision. First, we account for the fact that symbolic execution of expression DAGs with numerous reconvergent paths—commonly found in applications like FFTs and iterative solver expressions (see Figure~\ref{fig:gradual-abstraction})—tends to cause exponential growth in expression size. To mitigate this, we incorporate the fanout of a node (i.e., the number of consumers of the same expression value) into a formula (Equation~\eqref{eq:informtion}), which will be detailed shortly. Second, we recognize that each abstraction step involves a query to a global optimizer. Delaying abstractions too long can overwhelm the optimizer, creating a bottleneck. While this may suggest a need for earlier abstraction, premature abstraction risks losing variable correlations, which can degrade the accuracy of error bounds. To address this trade-off, we introduce the concept of an abstraction window, which bounds the abstraction height (Equation~\eqref{eq:select-height}). These considerations are formalized using concepts derived from Shannon’s work on information theory~\cite{Shannon1948}, specifically the notions of information content and entropy.

The information content, $I(n,h)$, of a node ($n$) at height $h$ in the Abstract Syntax Tree (AST) serves as a useful relative measure for \satire. Unlike the probabilistic measure used in Shannon's original work, this measure is tailored to \satire's context. Here, $H$ represents the full height of the AST, and $0\leq h\leq H$ denotes the distance of the node from the root. This concept is formalized in Equation~\eqref{eq:informtion}, which aids in identifying cut points for abstraction at candidate nodes $n$:

\begingroup
\small
    \begin{equation}
        \begin{split}
            I(n,h) = -\log(h/H) \cdot (fanout(n))
        \end{split}
        \label{eq:informtion}
    \end{equation}
\endgroup

A node at the root (output node) of the AST does not require abstraction and therefore contributes no meaningful information. Conversely, nodes farther from the root i.e. higher fanout are better candidates for abstraction. The measure $I(n,h)$ effectively captures this crucial information.

Next, we define the cost function as an information entropy measure, analogous to the expectation of information in Shannon's work. In \satire, all nodes at a selected height are abstracted, as illustrated in Figure~\ref{fig:gradual-abstraction}, which demonstrates two abstraction steps at a height of 2. Let $C(h)$ denote the cost function in this context, as defined in Equation~\eqref{eq:entrophy}, where $N(h)$ represents the set of all nodes at height $h$. According to this formula, the terms $h/H$ and $-\log(h/H)$ act in opposition, favoring $h$ values roughly ``midway'' along the AST:


\begingroup
\small
    \begin{equation}
        \begin{split}
            C(h) = \sum_{n_i \in N(h)}\left ( -\dfrac{h}{H}\cdot \log(h/H)
                                         \right ) \cdot fanout(n_i)
        \end{split}
        \label{eq:entrophy}
    \end{equation}
\endgroup
\noindent 

In \satire, an
  {\em abstraction window}, define by a pair $[H_1, H_2]$,
  bounds candidate abstraction heights, balancing expression sizes and variable correlations,
  as captured by Equation$~\eqref{eq:select-height}$:
\begingroup
\small
    \begin{equation}
        \begin{split}
            {\mathcal H} = \argmax_{H_1 \leq h \leq H_2} \sum_{n_i \in N(h)} \left ( -\dfrac{h}{H_2}\cdot \log(h/H_2)
                                         \right ) \cdot fanout(n_i)
        \end{split}
        \label{eq:select-height}
    \end{equation}
\endgroup

Here, ${\mathcal H}$ represents the selected abstraction height. As noted in~\cite{2020_Das}, the benefits of abstraction are significantly greater for nonlinear benchmarks compared to linear benchmarks. This distinction is not easily quantified by any equation and relies heavily on user judgment.

Our abstraction heuristic is not designed to be "optimal" in any specific sense. Instead, it aims to strike a practical balance between several competing factors that influence its effectiveness, while remaining fast and straightforward to implement. The efficacy of abstraction depends on various factors, including expression sizes, the degree of non-linearity, the extent of variable correlation loss, the execution time for each optimizer call, and more. Among these, our implementation prioritizes considerations such as sub-expression sizes, node fanouts, and variable correlations as the primary drivers of the heuristic.

==> Abstractions/files/fixed_depth_abstractions.tex <==
% \noindent{\bf Comparison with Fixed Depth Abstraction:\/}
\subsection{Comparison with Fixed Depth Abstraction}

Table~\ref{tab:fixed-depth} presents 
the error bounds and execution times 
for fixed abstraction depths across three examples: 
FFT, Lorenz70, and Scan. 
%
These examples highlight distinct and often competing aspects of abstraction. For the Scan example, tight error bounds can be achieved even with small abstraction depths, as variable correlation losses are minimal. 
%
In such cases, smaller abstraction depths that result in better overall runtime are preferred.

In contrast, FFT demonstrates a different behavior. 
Larger abstraction depths lead to tighter error bounds but with diminishing returns beyond a certain point, while execution time continues to increase. 
%
Rather than requiring users to identify this critical depth through trial-and-error, \satire's abstraction window mechanism allows users to specify a range of depths. For instance, a window of (10, 20) yields a bound of 4.52e-13 with an execution time of just 17 seconds. %
This approach eliminates the need for impractical manual tuning and ensures near-optimal performance.

While it may be tempting to treat \satire's global optimizer as a black box, 
doing so can severely degrade performance. 
%
For example, 
optimizer queries involving 2K operators complete in 26 seconds, 
whereas queries with 24K operators take 4,450 seconds - 
exhibiting near-exponential growth. 
%
Non-linear benchmarks are particularly sensitive to runtime increases, 
as their path-strength derivatives are symbolic expressions (in contrast to linear benchmarks, 
where derivatives are constants). 
%
This creates a dual source of expression complexity: 
forward symbolic expressions and path-strength derivatives. 
%
At shallow abstraction depths, forward expressions are small while derivatives are large; 
at greater depths, the reverse is true. 
Thus, abstractions applied midway through the expression tree yield the best results, 
balancing the complexity of forward and derivative expressions.

In our experiments (Table~\ref{tab:fixed-depth}), Lorenz70 illustrates the challenges posed by nonlinear benchmarks. 
%
At an abstraction depth of 19, error expressions overwhelm the optimizer, with each query taking hours to complete. 
%
In such cases, heuristic-based abstraction parameters help guide \satire effectively. Notably, the upper and lower bounds of the abstraction window specified by the user serve only as hints. 
%
\satire dynamically adjusts these bounds to manage large expression complexities. For instance, when Lorenz70 was tested with an abstraction window of (20, 40), \satire detected runtime saturation at a depth of 18 and automatically reduced the lower bound accordingly.

In summary, self-adjusting abstraction mechanisms in \satire eliminate the need for users to make specific and potentially suboptimal choices. This flexibility ensures robust performance across a wide range of benchmarks, enabling efficient and scalable error analysis.


%to enable queries that can be solved fast and efficiently.
%
%
%ranges.
%

%Table~\ref{tab:fixed-depth} summarizes the performance of
%fixed-depth abstraction applied to our study examples.
%

%
%Successive abstraction decisions
%will re-initialize starting with the
%20-40 range, but expected to be adjusted based on the corresponding sub-expression.
%
%
%In particular, giving a soft range rather than over-committing
%to a hardwired (but suboptimal) abstraction depth can
%pay-off dividends down the road.

\input{Abstractions(TACO25)/files/fixed_depth_table}

%It is clear that for unrolled stencil-type examples
%(Figure~\ref{fig:gradual-abstraction}), expression sizes
%grow very quickly, calling for abstractions.


==> Abstractions/files/fixed_depth_table.tex <==
\begingroup
\small
\begin{table}[ht]
\centering
\setlength\tabcolsep{2.5pt}
%\color{blue}
\begin{tabular}{ccccccc}
\toprule
\multirow{3}{*}{Fixed Depth} & \multicolumn{6}{c}{Examples} \\
\cmidrule(lr){2-7}
& \multicolumn{2}{c}{FFT} & \multicolumn{2}{c}{Lorenz70} & \multicolumn{2}{c}{Scan} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
				 & err 		& \shortstack[1]{Exec \\Time}			 & err		& \shortstack[1]{Exec \\Time} 			& err 		& \shortstack[1]{Exec \\Time}  \\
%lorenz20: x	 & 1.16e-14 & \multirow{3}{*}{12s}	 & 1.19e-14 & \multirow{3}{*}{519s} 	& 1.14e-14  & \multirow{3}{*}{528s}  \\
8	& 4.34e-13 & 14 & 1.12e-11 & 88 & 9.38e-13 & 24  \\
9 	& 3.98e-13 & 17 & 1.05e-12 & 45 & 9.38e-13 & 18 \\
10 	& 4.44e-13 & 18 & 2.58e-12 & 152 & 9.38e-13 & 22 \\
11	& 4.60e-13 & 18 & 4.56e-12 & 128 & 9.38e-13 & 35 \\
12	& 4.52e-13 & 18 & 5.58e-12 & 150 & 9.38e-13 & 49 \\
13	& 4.75e-13 & 24 & 1.70e-11 & 168 & 9.38e-13 & 61 \\
14	& 4.39e-13 & 24 & 5.91e-12 & 627 & 9.38e-13 & 78 \\
15	& 4.36e-13 & 28 & 7.31e-12 & 987 & 9.38e-13 & 93 \\
16	& 4.43e-13 & 42 & 7.90e-12 & 1220 & 9.28e-13 & 109 \\
17	& 4.18e-13 & 41 & 2.43e-12 & 3400 & 9.38e-13 & 131 \\
18  & 4.18e-13 & 47 & 7.93e-13 & 2041 & 9.38e-13 & 142 \\
%19	& 4.21e-13 & 70 & \multirow{7}{*}{NA} & \multirow{7}{*}{NA} & 9.38e-13 & 137 \\
19	& 4.21e-13 & 70 & \multicolumn{2}{c}{\multirow{3}{*}{NA}} & 9.38e-13 & 137 \\
20	& 4.08e-13 & 71 &          &      & 9.38e-13 & 140 \\
21	& 4.08e-13 & 68 &			&		& 9.38e-13 & 138 \\
%22	& 4.08e-13 & 104 &			&		& 9.38e-13 & 138 \\
%23	& 4.02e-13 & 101 &			&		& 9.38e-13 & 140 \\
%24	& 4.02e-13 & 99  &			&		& 9.38e-13 & 141 \\
%25	& 4.02e-13 & 143 &			&		& 9.38e-13 & 138 \\
\end{tabular}
\caption{Error bounds and execution times for three examples obtained when performing abstrcations for a set of fixed depth values}
\label{tab:fixed-depth}
\end{table}
\endgroup


==> Background/TACO25-files/floating_point_expressions.tex <==
\noindent{\bf {Floating-Point Expressions}:\/}

Let $\mathscr{E}^A$ denote $\mathscr{E}$ under the mapping A. Similar to $\mathscr{E}$ we can view $\mathscr{E}^A$ as a function $\lambda x.\mathscr{E}^A$ applied to an \emph{N-dimensional} float-valued vector $x.\mathscr{E}^A$. For instance, in the example above with $\mathscr{E}=x+y$ with mapping $A^\mathscr{E} = {(0, \epsilon_{32}), (1, \epsilon_{64}), (2, \epsilon_{32})}$, when we have x and y as real-valued inputs, x gets \emph{rounded more} and y gets \emph{rounded less} before the addition operation is carried out.

==> Background/TACO25-files/global_optimizer.tex <==
\noindent{\bf {Global Optimizers}:\/}
\subsection{Global Optimizers}

Gelpia is a global optimizer that uses a cooperative, interval-arithmetic branch-and-bound algorithm. It rigorously finds an upper bound on the global maximum of a multivariate function over a given interval. This means that its result is guaranteed to be above the global maximum on the interval when evaluated using real arithmetic. Gelpia is a cooperative solver in the sense that it concurrently runs fast, approximate algorithms to find local maxima, which inform the IBBA of new lower bounds.

==> Bound_Optimization/results-table.tex <==
\begingroup
\small
\begin{table}[htbp]
\centering
%\makebox[0pt][c]{\parbox{0.6\textwidth}{%
%\begin{minipage}[b]{0.7\hsize}
\begin{tabular}{cccc}
\toprule
\multirow{2}{*}{Benchmarks} &  \multicolumn{2}{c}{Absolute Error} & \multirow{2}{*}{\shortstack[l]{Num \\OPs}}\\
\cmidrule(lr){2-3} 
& {\satire} & {FPTaylor}  &  \\
\midrule
exp1x\_32			&		 \tb{\bf 1.12e-06}	& \tb{6.15e-06}   	&	5 	\\
\tb{doppler1}			&		 \tb{3.19e-13} 	& \tb{\bf 1.29e-13} & 10 \\
carbonGas			&		 \tb{\bf 4.13e-09}	& \tb{6.08e-09}  		&	21	\\
turbine3			&		 \tb{\bf 6.58e-15}  & \tb{1.06e-14}		 	&	23	\\
triangle			&		 \tb{\bf 2.50e-14}	& \tb{3.12e-14}		 	&	14	\\
rigidBody2			&        \tb{\bf 1.99e-11}  & \tb{3.61e-11}			&	17	\\
predatorPrey		&		 \tb{\bf 8.27e-17}	& \tb{1.59e-16} 		&	12	\\
jetEngine			&		 \tb{\bf 6.55e-12}	& \tb{1.03e-11}  		&	35	\\
bspline3			&		 \tb{\bf 2.78e-17}	& \tb{7.86e-17}			&	7 	\\
dqmom				&		 \tb{\bf 5.0e-10}*	& \tb{3.45e-05}			&	35	\\
\end{tabular}
\caption{\label{tab:satire-fptaylor}Comparison of Results ({\bf bold-face} highlights better results, and * highlights
  a difference of more than an order of magnitude)}
%\end{minipage}
%}}
%\label{tab:satire-fptaylor}
\end{table}
\endgroup


==> Evaluation/CLUSTER21-eval.tex <==
\subsection{CLUSTER21-eval}

\noindent{{\bf Experimental Setup: }}
\seesaw is a Python based framework.
Its symbolic data types are derived from
{\tt Symengine}.
%
All benchmarks were executed using
Python-3.8.0
on a dual 14-core Intel Xeon CPU E5-2680v4 2.60GHz CPUs 
(total 28 cores) with 128GB of RAM.
%
The core analyses in \seesaw were executed without
multicore parallelism (same for \fptaylor and \precisa)
to obtain comparable timings (the global optimizer
Gelpia
% ~\cite{gelpia-github} 
may internally spawn multiple threads).
%
Gelpia was used in \fptaylor as well as in \seesaw in an identical manner.
%
Version v4.1406 of \fluctuat was used.

\noindent{\bf Benchmarks:}
%
% \begin{comment}
% \skcmt{Is there a meaningful grouping of benchmarks:
% with/without conditionals, geometry, PDEs, etc.?
% Also, how about number of static asnd dynamic operations, number of conditionals, etc.?
% Given we want to claim the benchmark suite as a contribution, such a table can be included and referenced here.}
% \end{comment}
%
Our benchmark suite covers a wide variety 
of examples with special focus on
cases involving floating-point expressions
impacting the control flow. Such algorithms
(common in computational geometry
% ~\cite{compgeo}
and collision detection problems
% ~\cite{realtime}
)
are typically designed under an assumption of computations being
performed in exact real arithmetic.
Given the
numerical and geometrical nature of these 
algorithms, they are particularly sensitive to 
numerical robustness problems. 
%
Additionally, we include benchmarks involving
convergence testing such as in partial differential equation solving,
Conjugate Gradient methods and Gram-Schmidt orthogonalization.
%
We have also ported additional existing benchmarks for straight-line
codes with and without branches from other tools suites such as
\precisa and \fptaylor.
%

Our evaluation of \seesaw
emphasizes the following key aspects that are important when analyzing
floating-point programs:
 
\begin{comment}
(1)~{\em Worst case error bounds:\/} We report the bounds on the maximum absolute
  roundoff error that can be observed
  at the program output(s).
  %
  This analysis does not suppress inputs that fall into
  instability regions
  (constraints are comprised of weakened predicates).\footnote{\seesaw also
  supports the option to suppress such inputs; keeping these inputs gives nearly
  the same---and more conservative---results.}

(2)~{\em Instability bound:\/} We 
  report the maximal potential
  output result-jump caused by instability.
  %
  Additionally, \seesaw can sweep across all potential instability sites
  and rank order the amount of result jump
  that can potentially be introduced at those sites.

  %\skcmtside{What does "at the output" mean?} due to control-flow deviations.
  
  %\item {\em Solver comparison:\/} A comparative study of the performance, accuracy, and 
  %complexity 
  %associated with different solvers
  %is reported.
  %%solver types ( their efficacy contributes eventually  to bound tightness )

(3)~{\em Empirical consistency and Statistical error bounds:\/}
%\seesaw delivers rigorous first-order
%  error bounds.
  %
  To empirically calibrate
  the tightness of our 
  error estimates,  we cross-checked it 
  through shadow value calculations 
  at higher precision over a million samples per benchmark.
  %
  Also, after obtaining a
  predicated expression representing rounding error,
  we  statistically  
%  we employ solvers to calculate the supremum of
%  this function.
  %It can also, in addition,
  sample this function over a population of intervals,
  thus providing an alternate view of the error unbiased by potential
  over-approximations that solvers can introduce.  
  
%  a million tests were administered within the specified input intervals,
%  employing uniform random sampling.
%
%  bounds by performing extensive empirical testing using shadow value evaluations \skcmtside{What is consistency here?}.
% (4)~{\em Statistical error bounds:\/}
% 
%   %
% 
%   %
%   However, this risks under-reporting
%   due to sample insufficiency.

%\noindent Each of these items is discussed next.\\[0.5em]
\end{comment}

\input{Evaluation/CLUSTER21-files/solver-discussion}


%\noindent{\bf Empirical consistency}
\input{Evaluation/CLUSTER21-files/empirical-statistical}


%\noindent{\bf Instability analysis}
\subsection{\bf Instability analysis}
\input{Evaluation/CLUSTER21-files/instability}
\input{Evaluation/CLUSTER21-files/results-comp-table2}



%\noindent{\bf Comparative analysis:\/}
\subsection{\bf Comparative analysis}
In Table~\ref{tab:tools-compare-conds} we present comparative results 
for \seesaw, \precisa and \fluctuat for benchmarks containing
straight-line codes with conditions.
%
Comparison is presented for 
the total execution time, 
absolute error bounds and 
the bounds obtained on the output instability.
%
We report statistics obtained when using the `Preconditioned Optimizer'
solver type for \seesaw. 
%

We observe that while \precisa obtains better runtimes
in few of the benchmarks in comparison to \seesaw,
it is more efficient only for smaller
examples (it times out on many of \seesaw's larger examples).
%
In contrast, \seesaw obtains tight
error bounds for all benchmarks except in one (Barycentric)\footnote{These bounds get tightened when used
with constrained solver options -- using Z3/Dreal with increased query limit}. 


\fluctuat reports the best execution times across this 
set of benchmarks.
%
This is one of the best aspects of \fluctuat which is designed to
handle larger pieces of codes.
%
\seesaw's focus is on scaling adequately while offering rigorous and tighter bounds.

In examples such as
Symmetric Schur (SymSchur) decomposition, \seesaw produces
bounds that are 2 orders of
magnitude tighter than obtained by \fluctuat, and 10 orders of magnitude tighter than
produced by \precisa.
%
\seesaw is able to handle larg and complex benchmarks
with thousand of operators
and multiple conditionals nests.

%
%%\textcolor{red}{Fig.~\ref{fig:memory-profile} compares the memory consumption of \seesaw
%and \precisa for three benchmarks.}

%\subsubsection{\precisa}
%\subsubsection{\fluctuat}
%\subsubsection{\fptaylor}


%\begin{figure*}[h]
%  \centering % <-- added
%\begin{subfigure}{0.3\textwidth}
%\includegraphics[width=\linewidth]{graphs/mem-prof/barycentric-prec.pdf}
%\caption{Barycentric (\precisa)}
%\label{fig:1}
%\end{subfigure}\hfil % <-- added
%\begin{subfigure}{0.3\textwidth}
%\includegraphics[width=\linewidth]{graphs/mem-prof/gram-schmidt-prec.pdf}
%\caption{Gram-Schmidt (\precisa)}
%\label{fig:2}
%\end{subfigure}\hfil % <-- added
%\begin{subfigure}{0.3\textwidth}
%\includegraphics[width=\linewidth]{graphs/mem-prof/SpherePoint-prec.pdf}
%\caption{SpherePoint (\precisa)}
%\label{fig:3}
%\end{subfigure}
%%\begin{subfigure}{0.24\textwidth}
%%\includegraphics[width=\linewidth]{graphs/mem-prof/jet-prec.pdf}
%%\caption{Jetengine (\precisa)}
%%\label{fig:4}
%%\end{subfigure}
%
%\medskip
%\begin{subfigure}{0.3\textwidth}
%\includegraphics[width=\linewidth]{graphs/mem-prof/barycentric-sat.pdf}
%\caption{Barycentric (\seesaw)}
%\label{fig:5}
%\end{subfigure}\hfil % <-- added
%\begin{subfigure}{0.3\textwidth}
%\includegraphics[width=\linewidth]{graphs/mem-prof/gram-schmidt-sat.pdf}
%\caption{Gram-Schmidt (\seesaw)}
%\label{fig:6}
%\end{subfigure}\hfil % <-- added
%\begin{subfigure}{0.3\textwidth}
%\includegraphics[width=\linewidth]{graphs/mem-prof/SpherePoint-sat.pdf}
%\caption{SpherePoint (\seesaw)}
%\label{fig:7}
%\end{subfigure}
%%\begin{subfigure}{0.24\textwidth}
%%\includegraphics[width=\linewidth]{graphs/mem-prof/jet-sat.pdf}
%%\caption{Jetengine (\seesaw)}
%%\label{fig:8}
%%\end{subfigure}
%\caption{Memory Consumption comparison of three benchmarks for \precisa and \seesaw}
%\label{fig:memory-profile}
%\end{figure*}

%***>

We ran a memory profiler on the benchmarks when running both \precisa
and \seesaw.
%
Memory profiling of \seesaw and \precisa over Barycentric,
Gram-Schmidt and Spherepoint revealed that \seesaw had a
consistent memory usage, averaging 80MB over the entire execution.
%
\precisa's memory requirements went up from 150 MB
for Barycentric to 4GB (spiking to over 8GB)
for Gram-Schmidt, and 1GB to 5GB for Spherepoint,
terminating in both cases.

%% move straight-line code discussion to appendices
%In Table~\ref{tab:tools-compare-noconds},

We also performed a tool comparison
amongst \seesaw, \precisa, \fptaylor and \fluctuat
to ascertain performance consistency over straight-line programs without conditionals. 
%
\precisa obtains better execution times in about 50\% of the cases in which
it completes, particularly those with few dozen operators. However, for large
straight-line codes ($>$100 operators), both \precisa and \fptaylor run into scalability issues.
\seesaw performs consistently well, in execution speed and bound tightness across all these benchmarks and produces the tightest bounds.
%
\fluctuat has the best overall execution speed.
%
However, it bottlenecks for larger and complex programs
(the FFT benchmark in our case), quitting  unexpectedly.
%
As said earlier, \fluctuat is a closed-source tool whose
innards are unknown to us.
%
\fluctuat only reports the presence of instability jumps---not
its magnitude.

%--end

==> Evaluation/CLUSTER21-files/empirical-statistical.tex <==

\subsection{\bf Empirical testing and statistical profiling}
\begin{comment}
We perform shadow
value calculations to evaluate the empirical soundness and 
tightness of \seesaw{}-generated error bounds.
.... value This is done as a testing strategy
and remains external to \seesaw's framework. Additionally, since \seesaw
builds the full symbolic error expression, it can internally perform
statistical profiling on this expression itself.
\end{comment}
%
To empirically calibrate
  the tightness of our
  error estimates,  we cross-checked it
  through shadow value calculations
  at higher precision over a million samples per benchmark.
  %
  Also, after obtaining a
  predicated expression representing rounding error,
  we  statistically
%  we employ solvers to calculate the supremum of
%  this function.
  %It can also, in addition,
  sample this function over a population of intervals,
  thus providing an alternate view of the error unbiased by potential
  over-approximations that solvers can introduce.

Column `shadow profiling' in Table~\ref{tab:seesaw-solver-compare}
summarizes
the results of the empirical testing.
%
\seesaw's bounds were 
found to be always conservative and in many case within the same order of
magnitude of the observed empirical bound while being on average no worse than two orders of magnitude across all solver types
(except in specific cases of the basic Optimizer, which
being oblivious to the domain constraints,
may result in `inf').

%
\begin{comment}
While rigorous error
bounds are essential, 
in practice for distribution of specific inputs, 
they often seem to run the risk of incorporating
over-approximations introduced by solvers oblivious
of the input distributions.
%
%While rigorous error
%bounds are essential, in practice, for distributions of specific inputs, the
%rigorous bounds might seem to be large over-approximations while 
%shadow-value evaluations for specific inputs are expensive with a large additional memory requirement.
However, obtaining the exact error profile using shadow
value evaluations  is expensive due to additional memory resource requirement.
%
%\seesaw's support for statistical profiling of the symbolic error expression
%while also generating the rigorous bounds can provide valuable insights to inform the user of the error distribution.
%
%
\end{comment}
%
\begin{comment}
\end{comment}


Instead of performing global optimization of
the symbolic error expression, one can also
statistically sample it.
%
This provides a reasonable view of the underlying error
symbolic expression unaffected by overapproximations introduced by optimizers.
%
A large variation between rigorous worst-case error bound and sampled error bound
during statistical evaluation can provide valuable insight to the user---especially
if the worst-case is caused by a few outlier values.
%
In particular, the bounds obtained through sampling the error expressions must lie 
between the rigorous worst-case bounds and the exact runtime error on concrete data points.
%
This is because the error expressions themselves are over-approximations of
true runtime rounding errors. 
%
The difference between ``Prof Error Expr'' and ``Shadow profiling''
captures the amount by which our rigorous error analysis tends to be
conservative.
%
In almost all cases, the worst-case rigorous bound is within one order of magnitude
of the shadow value error bound.


%scenarios that cause the bloating in the rigorous bounds.
%
%to tighten the intervals being explored or investigate
%the outlier scenarios that cause the bloating in the rigorous bounds.
%

In Table~\ref{tab:seesaw-solver-compare},
column `Prof Error Expr' summarizes the
error estimates obtained by sampling the rigorous error expression bound.
%
Such sampling methods are often preferred to
shadow-value based error estimation, which requires
the same code to be instantiated in two different precisions---not always easy.
%
Our sampling methods follow a user-specified strategy (the default
being uniform sampling).






%\seesaw's tighness of bounds is attributed to 2 key attributes -- generating error expressions
%symbolically (that retains variable correlations) while also tracking  predicates along each program
%paths (enables domain constraint satisfiability check). 
%%
%We exploit this to enable statistical profiling of the error expression itself. 
%An immediate advantage of this technique is that it allows the user to peek into the profile
%of the error expression itself. In practice, when analyzing over large intervals, it is often the case
%that bloated error bounds are obtained while in practice the the bad corner cases rarely appears.
%A combined approach that informs the user about the maximum bound on absolute error ($E$) alongwith
%a statistical error($SE$ bound obtain through random sampling on the error expression itself 
%can be highly informative. For large $|E - SE|$, based on the application being analyzed the user may
%consider using the $SE$ value instead of $E$.
%%
%Note that built-up error expressions are already conservative since they are included in the guard of 
%{\tt abs(..)}. Hence the proximity of $SE$ to $E$ or shadow execution error ($SHE$) gives an indication into the
%nature of uncertainity of the code. 
%\begin{compactitem}
%\item {$SE$ is closer to $E$ but away from $SHE$:\/}   This informs large instability possible .
%\item {$SE$ is closer to $SHE$ but away from $E$:\/}   This implies unlikely by potential corner cases  lurking around.
%\adcmt{will discuss}
%\end{compactitem}
%Unlike shadow value 
%evaluation, this does not requires additional data structures -- however requires increased execution time
%due to statistical probing of the error expressions during the analysis.
%In Table~\ref{fig:seesaw-compare-solver}, column `Prof Error Expr' summarizes the values
%obtained using statistical sampling of the error expressions of the listed benchamrks.



==> Evaluation/CLUSTER21-files/instability.tex <==
We report the maximal potential
  output result-jump caused by instability.
  %
  Additionally, \seesaw can sweep across all potential instability sites
  and rank order the amount of result jump
  that can potentially be introduced at those sites.

While \seesaw's CCG generation facilitates
obtaining guarded path
constraints identifying valid program paths,
the path conditions may end up containing many
atomic inequalities containing large floating-point
expressions.
%
We rigorously analyze each of these Boolean predicates
involved in path conditions
and weaken each individual constraints
by including the instability region (``gray zone'') introduced due to roundoff
errors using the $wexpr$ rule in Listing ~\ref{lst:expression-weakening}.
%
Suppose $P$ represents the original atomic inequality
and $P^\prime$ denotes the weakened constraint obtained by `weakening' $P$ to include the rounding error. 
%
Under this transformation, $(P^\prime \wedge \lnot P^\prime)$ does not
evaluate to `False'. 
%
Instead, it identifies exactly the instability region in which the real execution
and the floating-point executions may diverge and cause instability.
%
%For example consider the simple
%case of $P: (x_1 - x_2) < 0.4$ and consequently $\lnot P : (x_1 - x_2) \geq 0.4$. Post-widening for
%a round-off error of say $0.01$, we get
%$P^\prime : (x_1 - x_2) < 0.4 + 0.01$, and $\lnot P: (x_1 - x_2) \geq 0.4 - 0.01$. 
%%
%Thus, we obtain  $P^\prime \wedge \lnot P^\prime : 0.39 \leq (x_1 - x_2) < 0.41$ -- yielding the
%exact instability region.
%

For a Boolean predicate
composed of many such inequalities, obtaining the cover for the combined instability region is 
in general non-trivial.
%
However, applying our {\em predicate weakening} approach to every atomic formula 
lends itself easily to
being incorporated in the most general manner
as part of the domain constraints.
%
 We solve for the function difference along each program path pairs in these instability regions 
and report the maximum for {\em instability quantification}.
%
The instability expression must be solved only for the instability constraint, 
otherwise it would be reporting bloated results over the entire interval as
shown in Table~\ref{tab:seesaw-solver-compare}.
%
In fact, we observe that the instability values become orders of magnitude tighter 
even with RealPaver guided PreConditioned intervals.
%

We also performed {\em empirical testing} to explore the input domain over randomly sampled 
 points to hit regions that trigger these instabilities.
%
In Table~\ref{tab:seesaw-solver-compare}, the last column lists the maximum instability jump
observed empirically using 10M tests per benchmark. The `-' entries did not hit any instability 
issues in our empirical tests.
%
\paragraph{{\bf Instability Bound Ranking}} \seesaw also reports the program path pairs that resulted in control flow divergence, and hence helping root-cause the source of maximum instability.
%
Although \seesaw reports the instability bound for the output node, it additionally
tracks the localized instability information at every internal
node of the conditional graph. It can yield additional analytical information on instability
by rank-ordering these bounds for every node and
extracting out the corresponding path predicates.
%
For example, consider the `Barycentric benchmark' which computes triples of
numbers that defines the position of a point in reference to a triangle containing the point.
In 
% ~\cite{realtime}
, the code for Barycentric coordinates requires evaluating two predicates.
We list the outer predicate $P1$ and the inner predicate as $P2$. Each of these predicates
makes decisions on the dot-product evaluation for pairs of sides of the reference triangle -- making them
susceptible to floating-point inaccuracies. \seesaw estimates an instability bound at the output of
$7.81$ if the control-flow traverses the instability region.
%
This analysis also exposes the predicates 
causing instability of internal nodes, giving a chance for the user to rewrite
these predicates in their code.
%
Table~\ref{tab:predorder} shows the rank-ordering of predicate combinations based on the maximum instability variations seen across
every internal and output node.

\begingroup
\small
\begin{table}[htbp]
\centering
\begin{tabular}{ccc}
\toprule
 Impacted Node & Predicates  &  Instability \\
 \midrule
	Internal &  $[P2^\prime, \lnot P2^\prime]$                                        &    215.2665   \\
	Internal &  \shortstack[1]{$[P2^\prime \wedge \lnot P1^\prime \wedge (P2^\prime \vee \lnot P2^\prime)$ ,\\ { $P1^\prime \wedge \lnot P2^\prime \wedge (P2^\prime \vee \lnot P2^\prime)]$}}       &   215.2665 \\
	{\bf Output}   &  $[P1^\prime, P2^\prime \wedge \lnot P1^\prime]$                              &     7.81  \\
	Internal &  $[\lnot P1^\prime \wedge \lnot P2^\prime, P2^\prime \wedge \lnot P1^\prime]$        &     2.74  \\
	Internal &  $[P1^\prime, \lnot P1^\prime \wedge \lnot P2^\prime \wedge (P2^\prime \vee \lnot P2^\prime)]$ &     0.058 \\
	%Internal &  $(P1^\prime, P2^\prime \wedge \lnot P1^\prime \wedge (P2^\prime \vee \lnot P2^\prime))$       &    172.12003   \\
 \end{tabular}
 \caption{\label{tab:predorder} Instability Bound Ranking: All impacted nodes are listed with the associated predicates and the instability values. In particular, the output node $\mathbf{res}$ is driven by 2 paths $\delta_1$ and $\delta_2$.} %-- evaluation.
 \end{table}
\endgroup



%\begingroup
%\small
%\begin{table}[htbp]
%\centering
%\begin{tabular}{ccc}
%\toprule
% Impacted Node & Predicates  &  Instability \\
% \midrule
%	Internal &  $(P2^\prime, \lnot P2^\prime)$                                        &    215.2665   \\
%	Internal &  $(P2^\prime \wedge \lnot P1^\prime \wedge (P2^\prime \vee \lnot P2^\prime), P1^\prime \wedge \lnot P2^\prime \wedge (P2^\prime \vee \lnot P2^\prime))$        &   215.2665 \\
%	{\bf Output}   &  $(P1^\prime, P2^\prime \wedge \lnot P1^\prime)$                              &     7.81  \\
%	Internal &  $(\lnot P1^\prime \wedge \lnot P2^\prime, P2^\prime \wedge \lnot P1^\prime)$        &     2.74  \\
%	Internal &  $(P1^\prime, \lnot P1^\prime \wedge \lnot P2^\prime \wedge (P2^\prime \vee \lnot P2^\prime))$ &     0.058 \\
%	%Internal &  $(P1^\prime, P2^\prime \wedge \lnot P1^\prime \wedge (P2^\prime \vee \lnot P2^\prime))$       &    172.12003   \\
% \end{tabular}
% \caption{\label{tab:predorder} Rank ordering of program paths based on instability evaluation.}
% \end{table}
%\endgroup



==> Evaluation/CLUSTER21-files/results-comp-table2.tex <==


%\begingroup
%\small
%
%	\begin{table*}[ht]
%	\centering
%  \begin{threeparttable}[t]
%	\begin{tabular}{ccccccccccccc}
%	\toprule
%	\multirow{2}{*}{Benchmarks}  &  \multirow{2}{*}{ OPs}  &  \multirow{2}{*}{ Conds} & \multicolumn{3}{c}{Abs Err} & \multicolumn{2}{c}{Exec Time[n]} & \multicolumn{3}{c}{Instability}  \\
%	\cmidrule(lr){4-6} \cmidrule(lr){7-8} \cmidrule(lr){9-11}
%	&             & &  {\seesaw} & {\precisa} & {\fluctuat} & {\seesaw} & {\precisa} & {\seesaw} & {\precisa} & {\fluctuat}  \\
%	\midrule
%	squareroot\tnote{b}      & 5    & 1  &  {\bf 1.77e-15}   & 4.2e-08  		& 1.11e-16 & 0.18s   & \bf{0.01s} & {\bf 2.68 }	& 2.70 & Y    \\ 
%	Barycentric\tnote{a}     & 83   & 2  &  {\bf 1.04e-15}   & 1.05e-14			& 2.67e-15 & {\bf 39s  }& 30m	& {\bf 3.93 }	& 4.26     & Y \\ 
%	SymSchur\tnote{a}        & 23   & 2  &  {\bf 4.02e-16}   & 1.3e-04  		& 2.21e-14 & {\bf 44s}		& 1750s		& {\bf 0.42 }	& 0.44     & Y \\ 
%	DistSinusoid\tnote{a}    & 32   & 2  &  {\bf 7.17e-06}   & NA           	& 1.27     & {\bf 23.4}     & --         &   {\bf 3.17}    & --       & Y \\   
%	Interpolator\tnote{c}    & 22   & 4  &  {\bf 1.47e-14}   & 3.07e-14 		& 1.51e-14 & 1.34s     		& \bf{0.1s } &	 {\bf 33.25}	& 225.0    & Y \\ 
%	Nonlin-interpol\tnote{c} & 6    & 1  &  {\bf 4.44e-16}   & 3.19e-14 		& 3.19e-14 & 1.12s     		& \bf{0.08s } &	 {\bf 2.9} 	& 101.01    & Y \\ 
%	EnclosingSphere\tnote{a} & 35   & 3  &  {\bf 4.41e-15}   & 1.67e-07			& 9.77e-15 & {\bf 7s }		& 9.8s 	 & {\bf 4.19}	& 9.18     & Y \\ 
%	Test2\tnote{a}           & 19   & 3  &  {\bf 7.65e-14}   & 3.53e-08 		& 6.55e-12 & 18s      		& \bf{0.6s } &	 {\bf 3.02 }	& 51.8     & Y \\ 
%	Closestpt2\tnote{a}      & 31   & 2  &  {\bf 9.15e-16}   & 4.24e-14 		& 4.06e-15 & {\bf 24s}		& 31s  		 	& {\bf 4.1  }	& 17.35    & Y \\ 
%	Cubicspline\tnote{c}     & 44   & 4  &  {\bf 2.66e-15}   & 1.33e-14 		& 1.99e-15 & 1.6s     		& \bf{0.4s}	 	& {\bf 16.0 }	& 27.0     & Y \\ 
%	Styblinski\tnote{c}      & 55   & 3  &  {\bf 7.32e-15}   & 4.04e-14 		& 2.91e-14 & {\bf 1.9s }	& 43s		 	& {\bf 0.01 }	& 93.4     & Y \\ 
%	SpherePt\tnote{a}        & 75   & 3  &  {\bf 1.76e-15}   &  --      		& 1.78e-14 & {\bf 40s  }	& -- 		 	& {\bf 0.365}	& --       & Y \\ 
%	lead-lag\tnote{b}        & 46   & 8  &  {\bf 2.93e-17}   &  --      		& 2.81e-16 & {\bf 11s  }	& -- 		 	& {\bf 0.04 }	& --       & Y \\ 
%	RayTracing\tnote{a}      & 119  & 8  &  {\bf 1.46e-15}   &  --      		& inf 	   & {\bf 331s }	& -- 		 	& {\bf 0.129}	& -- 	   & Y \\
%	EigenSphere\tnote{a}     & 334  & 13 &  {\bf 6.36e-16}   &  --      		& 2.078    & {\bf 438s }	& -- 		 	& {\bf 2.16 }	& --       & Y \\ 
%	Jacobi\tnote{a}          & 170  & 2  &  {\bf 1.15e-13}   &  --      		& 8.10e-12 & {\bf 138s }	& -- 		 	& {\bf 55.5 }	& --       & Y \\ 
%	Mol-Dyn\tnote{a}         & 179  & 6  &  {\bf 1.42e-15}   &  --      		& 6.21e-15 & {\bf --   }	& -- 		 	& --			& --       & Y \\
%	Gram-Schmidt\tnote{b}    & 471  & 19 &  {\bf 7.95e-17}   &  --      		& 1.44e-16 & {\bf 115s }	& -- 		 	& {\bf 0.02}	& --       & Y \\ 
%	Poisson\tnote{a}         & 2736 & 4  &  {\bf 1.0e-19 }   &  --      		&		   & {\bf 20s  }	& -- 		 &	& {\bf 0.97}	& --       & -- \\ 
%	CG\tnote{a}              & 210K & 4  &  {\bf 1.86e-18}   &  --      		&		   & {\bf 3142s}	& -- 		 &	& --			& --       & -- \\ 
%	\end{tabular}
%	\begin{tablenotes}
%		\item[a] New benchmarks introduced with \seesaw for conditional codes
%		\item[b] Benchmarks ported from FPBench
%		\item[c] Benchmarks ported from \precisa
%	\end{tablenotes}
%	\caption{\label{tab:tools-compare-conds} Comparative analysis with \precisa for codes with conditional branches. [n]:
%         \fluctuat took $< 0.1$ sec for all the rows.}
%  \end{threeparttable}
%	\end{table*}
%\endgroup


\begingroup
\small

	\begin{table*}[t]
	\centering
  \begin{threeparttable}[t]
	\begin{tabular}{crrrrrrrrrrrc}
	\toprule
	\multirow{2}{*}{Benchmarks}  &  \multirow{2}{*}{ OPs}  &  \multirow{2}{*}{ Conds} & \multicolumn{3}{c}{Absolute Error} & \multicolumn{2}{c}{Exec Time[n]} & \multicolumn{3}{c}{Instability}  \\
	\cmidrule(lr){4-6} \cmidrule(lr){7-8} \cmidrule(lr){9-11}
	&             & &  {\seesaw} & {\precisa} & {\fluctuat} & {\seesaw} & {\precisa} & {\seesaw} & {\precisa} & {\fluctuat}  \\
	\midrule
	squareroot\tnote{b}      & 5    & 1  &  1.77e-15   & 4.20e-08  		& {\bf 1.11e-16} & 0.18s   		& \bf{0.01s} 	& {\bf 2.68}	& 2.70 		& Y \\ 
	Barycentric\tnote{a}     & 83   & 2  &  {\bf 1.04e-15}   & 1.05e-14		& 2.67e-15 & {\bf 39.00s}	& 30.00m	& {\bf 3.93}	& 4.26  	& Y \\ 
	SymSchur\tnote{a}        & 23   & 2  &  {\bf 4.02e-16}   & 1.30e-04  		& 2.21e-14 & {\bf 44.00s}	& 1750.00s	& {\bf 0.02}	& 0.44  	& Y \\ 
	DistSinusoid\tnote{a}    & 32   & 2  &  {\bf 7.17e-06}   & NA           	& 1.27     & {\bf 23.40s} 	& --         	& {\bf 3.17}    & --    	& Y \\   
	Interpolator\tnote{c}    & 22   & 4  &  {\bf 1.47e-14}   & 3.07e-14 		& 1.51e-14 & 1.34s     		& \bf{0.10s} 	& {\bf 33.25}	& 225.00	& Y \\ 
	Nonlin-interpol\tnote{c} & 6    & 1  &  {\bf 4.44e-16}   & 3.19e-14 		& 3.19e-14 & 1.12s     		& \bf{0.08s} 	& {\bf 2.9} 	& 101.01	& Y \\ 
	EnclosingSphere\tnote{a} & 35   & 3  &  {\bf 4.41e-15}   & 1.67e-07		& 9.77e-15 & {\bf 7.00s}	& 9.80s 	& {\bf 4.19}	& 9.18     	& Y \\ 
	Test2\tnote{a}           & 19   & 3  &  {\bf 7.65e-14}   & 3.53e-08 		& 6.55e-12 & 18.00s      	& \bf{0.60s} 	& {\bf 3.02}	& 51.80     	& Y \\ 
	Closestpt2\tnote{a}      & 31   & 2  &  {\bf 9.15e-16}   & 4.24e-14 		& 4.06e-15 & {\bf 24.00s}	& 31.00s  	& {\bf 1.45}	& 17.35    	& Y \\ 
	Cubicspline\tnote{c}     & 44   & 4  &  {\bf 2.66e-15}   & 1.33e-14 		& 1.99e-15 & 1.60s     		& \bf{0.40s}	& {\bf 0.25}	& 27.00     	& Y \\ 
	Styblinski\tnote{c}      & 55   & 3  &  {\bf 7.32e-15}   & 4.04e-14 		& 2.91e-14 & {\bf 1.90s}	& 43.00s	& {\bf 0.01}	& 93.40     	& Y \\ 
	SpherePt\tnote{a}        & 75   & 3  &  {\bf 1.76e-15}   &  --      		& 1.78e-14 & {\bf 40.00s}	& -- 		& {\bf 0.36}	& --       	& Y \\ 
	lead-lag\tnote{b}        & 46   & 8  &  {\bf 2.93e-17}   &  --      		& 2.81e-16 & {\bf 11.00s}	& -- 		& {\bf 0.01}	& --       	& Y \\ 
	RayTracing\tnote{a}      & 119  & 8  &  {\bf 1.46e-15}   &  --      		& inf 	   & {\bf 331.00s}	& -- 		& {\bf 0.12}	& -- 	   	& Y \\
	EigenSphere\tnote{a}     & 334  & 13 &  {\bf 6.36e-16}   &  --      		& 2.07	   & {\bf 438.00s}	& -- 		& {\bf 2.16}	& --       	& Y \\ 
	Jacobi\tnote{a}          & 170  & 2  &  {\bf 1.15e-13}   &  --      		& 8.10e-12 & {\bf 138.00s}	& -- 		& {\bf 55.50}	& --       	& Y \\ 
	Mol-Dyn\tnote{a}         & 179  & 6  &  {\bf 1.42e-15}   &  --      		& 6.21e-15 & {\bf --   }	& -- 		& --		& --       	& Y \\
	Gram-Schmidt\tnote{b}    & 471  & 19 &  {\bf 7.95e-17}   &  --      		& 1.44e-16 & {\bf 115.00s}	& -- 		& {\bf 0.02}	& --       	& Y \\ 
	Poisson\tnote{a}         & 2736 & 4  &  {\bf 1.00e-19}   &  --      		& --	   & {\bf 20.00s}	& -- 		& {\bf 0.97}	& --       	& --\\ 
	CG\tnote{a}              & 210K & 4  &  {\bf 1.86e-18}   &  --      		& --	   & {\bf 3142.00s}	& -- 		& --		& --       	& --\\ 
	\end{tabular}
	\begin{tablenotes}
		\item[a] New benchmarks introduced with \seesaw for conditional codes
		\item[b] Benchmarks ported from FPBench
		\item[c] Benchmarks ported from \precisa
	\end{tablenotes}
	\caption{\label{tab:tools-compare-conds} Comparative analysis with \precisa for codes with conditional branches. [n]:
         \fluctuat took $< 0.1$ sec for all the rows. '-' denotes program timed out.}
  \end{threeparttable}
	\end{table*}
\endgroup


%	\midrule
%	%\multirow{16}{*}{\shortstack[1]{Codes with \\{Conditionals}}} & 
%	squareroot   & 5    & 1  &  6.1e-16    & 0.3s      & 2.68     & 4.2e-08   & 0.01s       & 2.68      \\
%	Test2        & 19   & 3  &  2.91e-14   & 18s       & 3.38     & 3.53e-08  & 0.6s        & 51.8      \\
%	Interpolator & 22   & 4  &  1.24e-14   & 0.8s      & 115.0    & 3.07e-14  & 0.1s        & 225.0     \\
%	SymSchur     & 23   & 2  &  8.64e-17   & 44s       &  0.42    & 1.3e-04   & 1750s       & 0.44      \\
%	Closestpt2   & 31   & 2  &  9.15e-16   & 24s       & 4.1      & 4.24e-14  & 31s         & 17.35     \\  
%	EncloSphere  & 35   & 3  &  2.01e-15   & 3s        & 9.125    &  1.67e-07 & 9.8s        & 9.18      \\
%	Cubicspline  & 44   & 4  &  2.66e-15   & 1.6s      & 16.0     & 1.33e-14  & 0.4s        & 27.0      \\
%	Styblinski   & 55   & 3  &  7.32e-15   & 1.9s      & 0.01     & 4.04e-14  & 43s         & 93.4      \\ 
%	SpherePt     & 75   & 3  &  1.76e-15   & 40s       & 0.365    &  NA       & NA          & NA        \\
%	lead-lag     & 46   & 8  &  2.93e-17   & 11s       & 0.04     &  NA       & NA          & NA        \\
%	Barycentric  & 83   & 2  &  1.34e-15   & 64s       &  3.93    & 1.05e-14  & 30m         & 4.26      \\
%	EigenSphere  & 334  & 13 &  6.36e-16   & 438s      & 2.16     &  NA       & NA          & NA        \\
%	Jacobi       & 170  & 2  &  1.15e-13   & 138s      & 55.5     &  NA       & NA          & NA        \\
%	Gram-Schmidt & 471  & 19 &  7.95e-17   & 115s      & 0.02     &  NA       & NA          & NA        \\
%	Poisson      & 2736 & 4  &  1.0e-19    & 20s       & 0.97     &  NA       & NA          & NA        \\
%	CG           & 210K & 4  &  1.86e-18   & 3142s     & --       &  NA       & NA          & NA        \\
%	%% FPTaylor suite straight line examples
%	\end{tabular}
%	\caption{\label{tab:tools-compare} Comparative analysis with Precisa for codes with conditional branches}
%	\end{table}
%\endgroup

%  \begingroup
%  \small
%  
%  	\begin{table*}[ht]
%  	\centering
%  	\begin{threeparttable}
%  	%\setlength\tabcolsep{1.5pt}
%  	\begin{tabular}{cccccccccc}
%  	\toprule
%  	\multirow{2}{*}{Benchmarks}  &  \multirow{2}{*}{ OPs}  & \multicolumn{2}{c}{\seesaw} & \multicolumn{2}{c}{\precisa} & \multicolumn{2}{c}{\fptaylor} & \multicolumn{2}{c}{\fluctuat}\\
%  	\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
%  	             & &  {Abs-Err} & {Exec-Time} & {Abs-Err} & {Exec-Time} & {Exec-Time} & {Abs-Err} & {Exec-Time} & {Abs-Err}   \\	
%  	\midrule
%  %	\multirow{9}{*}{Straight line  Codes} &
%  	%\multirow{9}{*}{\shortstack[1]{Codes without \\{Conditionals}}} & 
%  	predprey\tnote{a}     &	8		&  {\bf 1.99e-17}   & 0.1s			&  2.08e-16 & {\bf 0.02s}	&  1.59e-16   &  0.74s    &\multirow{14}{*}{< 0.1s} & 2.5e-16 \\
%  	doppler1\tnote{a}     &	10		&  {\bf 2.30e-14}   & 0.57s			&  2.08e-13 & {\bf 0.08s}	&  1.28e-13   &  1.95s    & & 3.9e-13 \\
%  	doppler2\tnote{a}     &	10		&  {\bf 4.51e-14}   & 0.55s			&  3.07e-13 & {\bf 0.07s}	&  2.38e-13   &  2.01	  & & 9.7e-13 \\
%  	doppler3\tnote{a}     &	10		&  {\bf 1.07e-14}   & 0.65s			&  9.5e-14  & {\bf 0.08s}	&  2.38e-13   &  2.01	  & & 1.5e-13 \\
%  	turbine3\tnote{a}     &	16		&  {\bf 3.04e-15}   & {\bf 0.27s}	&  1.82e-14 & 0.29s			&  1.05e-14   &  0.95     & & 6.99e-14\\
%  	sphere\tnote{a}       &	7		&  {\bf 2.78e-15}   & 0.14s			&  9.99e-15 & {\bf 0.01s}	&  7.64e-15   &  10.5s    & & 1.03e-14\\
%  	carbongas\tnote{a}    &	14		&  {\bf 3.84e-09}   & 0.13s			&  7.09e-09 & {\bf 0.02s}	&  6.07e-09   &  0.8s     & & 4.52e-08\\
%  	rigidbody2\tnote{a}   &	14		&  {\bf 1.22e-11}   & {\bf 0.14s}	&  3.64e-11 & 0.5s			&  3.60e-11   &  0.6s     & & 3.64e-11\\
%  	kepler0\tnote{a}      &	15		&  {\bf 3.47e-14}   & 0.61s			&  1.09e-13 & {\bf 0.35s}	&  7.47e-14   &  1.34s    & & 1.12e-13\\
%  	kepler1\tnote{a}      &	24		&  {\bf 1.19e-13}   & {\bf 0.62s}	&  4.03e-13 & 1.2s			&  2.86e-13   &  10s      & & 5.13e-13\\
%  	kepler2\tnote{a}      &	36		&  {\bf 7.28e-13}   & 1.42s			&  1.66e-12 & {\bf 0.49s}	&  1.57e-12   &  10.8s    & & 2.61e-12\\
%  	jetengine\tnote{a}    &	35		&  {\bf 5.21e-12}   & {\bf 1.6s }	&  1.79e-11 & 170s			&  1.02e-11   &  2.47s    & & 4.08e-08\\  
%  	lorenz40\tnote{b}  	  &	600		&  {\bf 8.22e-14}   & {\bf 48s  }	&  --       & --			&   --        &  --       & & 9.57e-14\\
%  	%lorenz70\tnote{b}     &	1050	&  {\bf 8.98e-13}   & {\bf 109s }	&  --       & --			&   --        &  --       & & \\
%  	Scan1024\tnote{b}     &	2036	&  {\bf 9.38e-13}   & {\bf 145s }	&  --       & --			&   --        &  --       & & 1.53e-12\\
%  	fft1024\tnote{b}      &	81K		&  {\bf 7.90e-13}   & {\bf 1948s}	&  --       & --			&   --        &  --       & -- & --\\
%  	%hartman6     & 190  &  1.29e-12   & 12s        &  4.67e-13 & 8m          &   1.60e-14  &  25s      \\
%  	\end{tabular}
%  	\begin{tablenotes}
%  		\item[a] Benchmarks ported from FPTaylor + also supported in PRECiSA
%  		\item[b] From a recent collection of large benchmark problem in~\cite{arxiv-satire}
%  	\end{tablenotes}
%  	\caption{\label{tab:tools-compare-noconds} Comparative analysis of \seesaw with Precisa and FPtaylor for straight line codes}
%  	\end{threeparttable}
%  	\end{table*}
%  \endgroup


==> Evaluation/CLUSTER21-files/solver-discussion.tex <==
\subsection{\bf Worst case error bounds}
\label{sec:solver-type}

%The advantage of \seesaw is that it is able to do path precise tracking
%of predicates leading to the program output. 
%
We report the bounds on the maximum absolute
  {\em roundoff error} that can be observed
  at the program output(s).
  %
  This analysis does not suppress inputs that fall into
  instability regions
  (constraints are comprised of weakened predicates).\footnote{\seesaw also
  supports the option to suppress such inputs; keeping these inputs gives nearly
  the same---and more conservative---results.}

We support
a basic {\em Optimizer} and a {\em Preconditioned Optimizer}.
The predicates defining
the function domains are
set to `True' in the basic Optimizer.
%
This allows us to
obtain a baseline where
we revert back to rectangular
domains encompassing the actual
function domains.
%
This is guaranteed to be a sound
(if quite loose) over-approximation.
%
To include constraints,
we have experimented 
with two SMT solvers,
namely Dreal and Z3,
that can
filter out boxes as needed
(for reasons
of space,
these results are not reported).
%
Owing to their wide spread use in Floating Point Error Analysis related projects
% ~\cite{rosa,dreal}
,
our choice of SMT solvers for handling non-rectangular domains in \seesaw were Z3 and Dreal.
%
In the Preconditioned Optimizer, we report results
from a second
approach
called
{\em Preconditioning}
(or ``paving'' using
RealPaver): 
we filter out invalid intervals a priori and
feed
smaller intervals that
contain the valid solution space.

\input{Evaluation/CLUSTER21-files/results-table1}

Table~\ref{tab:seesaw-solver-compare} summarizes the evaluation
of benchmarks involving straight-line codes with conditionals 
for the two solver types.
%
Across all benchmarks, the order of absolute error bounds reported are within
one order of magnitude for each of the solver type.
%
However, the basic Optimizer obtains near optimal answers with a
short execution time in most cases,
however trading off bound tightness.
%
This trade-off is more pronounced when
performing the {\em instability analysis}
because the order of the function jumps
are affected if solved without sufficiently tight
domain constraints.
%
We ran each solver with the same `timeout' parameter of 10
seconds per query (1000s of optimizer queries made).
%This allowed `Opt' to perform more interval subdivision per unit timeout, hence obtaining better throughput.
%


%% This paragraph discussion will be moved to appendices
\begin{comment} %-----------------
The constraint solver needs to perform
 more work per unit time in comparison to the basic optimizer
(requires solving SMT queries;
Table~\ref{tab:summary-smt}
lists the number of SMT calls made to obtain the final solution).
%
Not burdened by SMT queries,
`Opt' gets ``extra time'' to perform more interval subdivisions per unit
timeout window, hence obtaining better throughput.
%
In such cases,
the timeout for the individual queries can be increased to allow 
for an equivalent search space exploration.
%
In `Test2', when executed with the same timeout of 10s per query,
`OptC' returns a loose bound of 5.74e-14 whereas 'Opt' returns 3.12e-14.
Increasing the timeout to 60s
per query improve the OptC's answer to 3.43e-14 while `Opt' reveals
that it already has saturated.
%
The best answer 
of 2.91e-14 was obtained by `POpt' which was based on the paved boxes generated by
`RealPaver'. 
%

In fact, the immediate benefits of having 
a Preconditioned Interval set before invoking the optimizer is evident in 
over 80\% of the benchmarks -- leading to tighter bounds. 
%
For examples, in Styblinski, the bound tightens
by almost 50\% if intervals paved by RealPaver are provided to the optimizer 
instead of the initial domain of intervals.
%
`POpt' mostly outperforms the other solver types in combined merits of bound tightness,
execution speed and managing solver complexity.
%
\end{comment}
%%---------------------




%\paragraph{Three Solver types:\/} Table~\ref{tab:seesaw-solver-compare}  
%%-------------- Move to appendices -----------
\begin{comment}
\paragraph{Constraint solver:\/} For constraint solving, \seesaw 
provides interfaces to two SMT solvers:  (1) Dreal~\cite{dreal} and (2) Z3~\cite{z3}.
%
Z3 provides the guarantee of exact satisfiability or returning `unknown'
if it fails to prove a constraint unsatisfiable. 
%
In contrast Dreal's $\delta$-complete decision procedures weaken 
the constraint formula hence aiding in convergence and faster solution 
time.
%
Note that the $\delta$-weakened formula
may return $\delta$-sat or provably {\em unsat}. 
%
Hence, the following guarantees hold when solving with Dreal
\begin{compactitem}
	\item  for an unsatisfiable formula, Dreal's weakening may return `satisfiable',
	leading to an over-approximation.
%
	\item It may never return {\em unsat} if the original formula
is {\em satisfiable} -- thus ensuring never losing a solution
space, hence always guaranteeing a sound over-approximation in our usage.
\end{compactitem}

Our experiments show that Dreal and Z3 obtain the same answers to queries in
a majority of the cases (>90\%).
%
Furthermore,
we execute Dreal with an extremely small $\delta=$10e-15 to keep the answers tight.
%
However, Z3 took an average of 174s to complete in comparison to Dreal's 86s.
%
Thus, Z3 requires
a larger `timeout' value than when using Dreal due to a slower
search space exploration process.
%
However, if the user wishes to not compromise on $\delta$-weakening of the constraints, 
Z3 can obtain the tightest guarantees, albeit at the expense of larger execution times.
%



\begin{figure}
\centering
\begin{minipage}{0.55\textwidth}
  \includegraphics[width=0.8\textwidth,height=0.6\columnwidth]{figs/maxima}
  \caption{Variation in optimal solution based on domain constraints.}
  \label{fig:maxima}
\end{minipage}
\hfill
\begin{minipage}{0.4\textwidth}
\begin{tabular}{cc}
\toprule
Benchmark    &  \# SMT queries \\
\midrule
	Barycentric      &   1,071,868 \\
	Jacobi           &   57,754   \\
	Styblinski       &   13,807   \\
	SymSchur         &   17,048   \\
	Test2            &   33,871   \\
	EigenSphere      &   561,135  \\
	Mol-Dyn          &   122,360  \\
	JetApprox        &   9,314	 \\ 
	Gram-Schmidt     &   247,274  \\

\end{tabular}
\caption{\label{tab:summary-smt} Summary of SMT calls made}
\end{minipage}
\end{figure}




To re-emphasize the
value of having multiple options for solvers within \seesaw, we present 
Figure~\ref{fig:maxima}. It highlights the situation where the maxima pertaining to
the domain constraints is not really the global maxima. Using `Opt' will
result in bloated answers in such cases. For example, in a certain query (listed in appendix),
`Opt' returns 203.42; however, when guided by either Dreal or Z3, it return 7.38 as the
answer.

In our experiments, `POpt' performed the best,
and hence we will be using the numbers returned by `POpt' for 
comparative analysis in successive discussions.
\end{comment}
%%--------------------------


==> Evaluation/SC20-eval.tex <==
\subsection{SC20-eval}

\noindent{{\bf Tool Overview: }} Figure~\ref{fig:satire-flow}
provides an overview of the various stages of 
\satire's  execution.
%
\satire begins by reading-in a problem definition file 
in a simple syntax describing expressions and input intervals,
and also optional command line arguments for abstraction-specific
parameters.
%
Each symbolic variable is derived from the {\em var} datatype of
Symengine
% ~\cite{symengine}
.
%
First,
\satire builds the full abstract syntax tree (AST).
%
If abstraction is disabled,
\satire initiates Direct Solve that bypasses
abstraction,  attempting
to directly solve for the full error expression.
%
Otherwise, the abstraction loop is entered
with the specified abstraction window
(defaults to $[10,40]$, unless
the user overrides this choice).
%
All nodes at the heuristically
determined abstraction height $h$
(\S\ref{sec:abstractions})
are then abstracted by calling Direct Solve on
the set of selected candidate nodes
(denoted by the dashed line in figure~\ref{fig:satire-flow}.
%
Post abstraction, the abstracted nodes are mutated to become
free variables, with concrete function and error intervals.
%
An AST that reduces in height by $h$ is then
rebuilt.
%
If warranted, the process of abstraction continues
for the remaining AST; else
Direct Solve is invoked on the AST that remains
at this point.

\begin{figure}[h]
	\centering
    \includegraphics[width=0.5\textwidth, height=0.5\columnwidth]{Evaluation/SC20-figs/satire-flow.pdf}
  \caption{Overview of \satire}
  \label{fig:satire-flow}
\end{figure}

During Direct Solve,
\satire first invokes an expression builder to assign symbolic expression at each
node, conducting expression canonicalization
(\S\ref{sec:canonicalize}) in the process via the {\em expand}
functionality of Symengine.
%
Next, the Expression Builder performs a depth-first
traversal beginning from the set of root nodes
(\satire allows for solving multi-rooted expression DAGs).
%
It is followed by a
breadth-first traversal to obtain the {\em reverse mode symbolic derivatives}
(we have built this functionality as part of \satire).


Once both the symbolic
expression and derivative are available at a node,
\satire generates the corresponding symbolic error expression
contributed by the node to each DAG output,
aggregating these error expressions
in an accumulator held at the outputs.
%
The derivative evaluation and error generation are done in
synchrony
to avoid multiple traversals of the AST.
%
When the output node error accumulation is finished,
the results are fed 
to the global optimizer (Gelpia) to obtain its concrete error bound.


\noindent{{\bf Experimental Setup: }}
\satire is compatible with Python3, and
its symbolic engine is based on {\tt SymEngine}
% ~\cite{symengine}
.
%
All benchmarks were executed with Python3.8.0 version on a
dual 14-core Intel Xeon CPU E5-2680v4 2.60GHz CPUs system (total
28 processor cores) with 128GB of RAM.
%
%The comparative data
%for FPTaylor were generated on the same machine configurations.
%
To arrive at an objective comparison,
the core analysis algorithms were measured without any multicore parallelism
(both for FPTaylor and \satire).
%
The Gelpia solver (optimizer) does employ internal multithreading: we did not alter it
in any way when we used either FPTaylor or \satire.
%
All FPTaylor benchmarks used their specified data types.


Our main focus during evaluation will be the larger benchmarks, none
of which can be rigorously analyzed by other tools.
%
These are instantiated using the {\tt double precision} floating-point type.
%
For our empirical checks using shadow values, we employed
GCC's {\tt quadmath}.
%--end



%\begingroup
%\small
% \begin{table*}[ht]
% \centering
% \begin{threeparttable}[t]
%
%  \begin{tabular}{ccccccccccc}
%  \toprule
%  \multirow{2}{*}{Benchmarks} & \multirow{2}{*}{Num OPs} & \multicolumn{2}{c}{Direct Solve} & \multicolumn{2}{c}{Window-(10,20)} & \multicolumn{2}{c}{Window-(15,25)} & \multicolumn{2}{c}{Window-(20,40)} & \multirow{2}{*}{Empirical}\\
%
%  \cmidrule(lr){3-4}  \cmidrule(lr){5-6}  \cmidrule(lr){7-8}  \cmidrule(lr){9-10}
%
%  & & \shortstack[1]{Absolute \\{Error Bound}} & \shortstack[1]
%  {Execution \\Time\\ (secs)} & \shortstack[1]{Absolute \\{Error Bound}} & \shortstack[1]{Execution \\Time\\(secs)} & \shortstack[1]{Absolute \\{Error Bound}} & \shortstack[1]{Execution \\Time\\(secs)} & \shortstack[1]{Absolute \\{Error Bound}} & \shortstack[1]{Execution \\Time \\ (secs)} \\
%  \midrule\\
%  %\midrule
%  lorenz20(y) & 300 & NA & NA & 2.53e-14 & 13 & 2.54e-14 & 519 & 2.51e-14 & 528 & 3.5e-15 \\
%  lorenz40(y) & 600 & NA & NA & 1.93e-13 & 30 & 1.95e-13 & 1131 & 1.88e-13 & 1192 & 4.10e-14\\
%  lorenz70(y) & 1050 & NA & NA & 2.67e-10 & 50 & 1.05e-10 & 2050 & 1.05e-10 & 2079 & 1.01e-14\\
%  %\midrule
%  {Scan(1024pt)} & 2K & 1.88e-12 & 137  & 1.88e-12 & 137  & 1.88e-12 & 136  & 1.88e-12 & 137 & 5.82e-13 \\
%  {Scan(4096pt)} & 8K & 9.32e-11 & 2786  & 9.32e-11 & 13  & 9.32e-11 & 2837  & 9.32e-11 & 2859 & 2.7e-13 \\
%  %\midrule
%  {FFT-1024pt} & 81K & 7.98e-13 & 154 & 9.25e-13 & 105 & 8.89e-13 & 44 & 7.98e-13 & 154 & 6.09e-15 \\
%  {FFT-4096pt} & 393K & 3.64e-12 & 2706 & 4.05e-12 & 320 & 3.85e-12 & 169 & 3.63e-12 & 2429 & 1.05e-15 \\
%  %\midrule
%  %\multirow{11}{*}{\shortstack[1]{Finite Difference \\{Stencils}}} 
%   %H1\tablefootnote{\label{fpdlabel}These benchmarks were ported from ~\cite{fpd}} & 392K & NA & NA & 2.22e-14 & 2108 / 274 s & 2.22e-14 & 4192 / 692 s & 2.22e-14 & 10579 / 2615 s \\
%   H1\tnote{a} & 392K & NA & NA & 2.22e-14 & 2108 / 274 & 2.22e-14 & 4192 / 692 & 2.22e-14 & 10579 / 2615 & 4.56e-16 \\
%   H2\tnote{a} & 393K & NA & NA & 3.88e-14 & 2580 / 281 & 3.88e-14 & 4186 / 694 & 3.88e-14 & 10480 / 2603 & 7.55e-16 \\
%   H0\tnote{a} & 393K & NA & NA & 1.11e-13 & 1334 / 280 & 1.11e-13 & 3784 / 697 & 1.11e-13 & 10472 / 2597 & 1.49e-15 \\
%   P1\tnote{a} & 436k & NA & NA & 4.52e-14 & 882 / 234  & 4.52e-14 & 1346 / 265 & 4.52e-14 &  2445 / 966  & 3.6e-15 \\
%   P2\tnote{a} & 436k & NA & NA & 4.53e-14 & 1134 / 161 & 4.53e-14 & 1577 / 456 & 4.53e-14 &  2428 / 942  & 3.37e-15 \\
%   P0\tnote{a} & 436k & NA & NA & 1.50e-13 & 606 / 180  & 1.50e-13 & 1225 / 458  & 1.50e-13 & 2435 / 1114 & 1.28e-14 \\
%   C1\tnote{a} & 436k & NA & NA & 1.25e-14 & 2157 / 1186 & 1.25e-14 & 4312 / 3038 & 1.25e-14 & 10875 / 7969 & 8.96e-15 \\
%   C2\tnote{a} & 436k & NA & NA & 1.25e-14 & 2582 / 1277 & 1.25e-14 & 4303 / 3410 & 1.25e-14 & 10766 / 8143 & 2.10e-16 \\
%   C0\tnote{a} & 436k & NA & NA & 1.11e-13 & 1593 / 914  & 1.11e-13 & 4164 / 2827 & 1.11e-13 & 10839 / 7946 & 1.80e-15\\
%   Advection & 453k & 2.22E-13 & 2672 & 2.22e-13 & 2667 / 1223 & 2.22e-13 & 2703 / 1297 & 2.22e-13 & 2672 / 1319 & 1.4e-15 \\
%   FDTD & 192k & 7.45e-13 & %2.5 hrs & -- & -- & -- & -- & -- & -- \\
%                             9000 & -- & -- & -- & -- & -- & -- & 1.48e-15 \\
%  %Stencils & H1 & 393K & NA & NA & 2.22e-14 & 2108 s & 2.22e-14 & 4192 s & 2.22e-14 & 10579 s \\
%  %\midrule
%  matmul-64x64 & 520K & 9.51e-13 & 65 & 9.51e-13 & 58 & 9.51e-13 & 55 & 9.51e-13 & 54 & 3.82e-13 \\
%  matmul-128x128 & 4177K & 3.72e-12 & 833 & 3.72e-12 & 1189 & 3.72e-12 & 556 & 3.72e-12 & 527 & 1.28e-13 \\
%  %\midrule
%  {Tensor contraction} & 1530K & NA & NA & 4.55e-13 & 6309 & 4.55e-13 & 55902 & 4.55e-13 & 59640 & --\\
%  {Tensor contraction}\tnote{b} & 1530K & NA & NA & 1.57e-19 & 1473 & 1.57e-19 & 953 & 1.57e-19 & 752 & NA \\
%  %\midrule
%  %{Tref} & 22K & 1.16e-14 & 3 s & 1.55e-09 & 60 s & 3.38e-10 & 57 s & 1.25e-09 & 32 s \\
%  {CG-Arc}\tnote{b} & 211K & 1.78e-19 & 280 & 1.23e-17 & 2291 & 1.68e-17 & 1032 & 1.54e-17 & 3866 & NA\\
%  {CG-Pores}\tnote{b} & 45K & 5.34e-05 & 9 & -- & -- & -- & -- & -- & -- & NA \\
%  %\midrule
%	\end{tabular}
%	\begin{tablenotes}
%	\item[a] Benchmarks ported from ~\cite{fpd}
%	\item[b] Benchmarks analyzed over degenerate intervals
%	\end{tablenotes}
%	\caption{\label{tab:satire-results} Satire evaluated worst case absolute error bounds and execution time on larger benchmarks. }
% \end{threeparttable}
% \end{table*}
%\endgroup


\begingroup
\small
 \begin{table*}[ht]
 \centering
 \begin{threeparttable}[t]
\setlength\tabcolsep{2.5pt}
  \begin{tabular}{cccccccccc}
  \toprule
  \multirow{2}{*}{Benchmarks} & \multirow{2}{*}{Num OPs} & \multicolumn{2}{c}{Direct Solve} & \multicolumn{2}{c}{Window-(10,20)} & \multicolumn{2}{c}{Window-(15,25)} & \multicolumn{2}{c}{Window-(20,40)} \\

  \cmidrule(lr){3-4}  \cmidrule(lr){5-6}  \cmidrule(lr){7-8}  \cmidrule(lr){9-10}

  & & \shortstack[1]{Absolute \\{Error Bound}} & \shortstack[1]
  {Execution \\Time\\ (secs)} & \shortstack[1]{Absolute \\{Error Bound}} & \shortstack[1]{Execution \\Time\\(secs)} & \shortstack[1]{Absolute \\{Error Bound}} & \shortstack[1]{Execution \\Time\\(secs)} & \shortstack[1]{Absolute \\{Error Bound}} & \shortstack[1]{Execution \\Time \\ (secs)} \\
  \midrule\\
  %\midrule
  lorenz20(y) & 300 & NA & NA & \tb{1.25e-14} & 14 & \tb{1.25e-14} & 519 & \tb{1.24e-14} & 528 \\
  lorenz40(y) & 600 & NA & NA & \tb{9.11e-14} & 29 & \tb{9.33e-14} & 1131 & \tb{9.02e-14} & 1192 \\
  lorenz70(y) & 1050 & NA & NA & \tb{1.06e-12} & 50 & \tb{8.14e-13} & \tb{2088} & \tb{8.14e-13} & \tb{2150} \\
  %\midrule
  {Scan(1024pt)} & 2K & \tb{9.38e-13} & \tb{141}  & \tb{9.38e-13} & \tb{141}  & \tb{9.38e-13} & \tb{141}  & \tb{9.38e-13} & \tb{141}  \\
  {Scan(4096pt)} & 8K & \tb{4.66e-11} & \tb{2822}  & \tb{4.66e-11} & 13  & \tb{4.66e-11} & 2837  & \tb{4.66e-11} & 2859  \\
  %\midrule
  {FFT-1024pt} & 81K & \tb{3.98e-13} & \tb{171} & \tb{4.52e-13} & \tb{17} & \tb{4.36e-13} & \tb{28} & \tb{3.98e-13} & \tb{171} \\
  {FFT-4096pt} & 393K & \tb{1.82e-12} & \tb{2581} & \tb{2.02e-12} & \tb{68} & \tb{1.935e-12} & \tb{106} & \tb{1.82e-12} & {2576} \\
  %\midrule
  %\multirow{11}{*}{\shortstack[1]{Finite Difference \\{Stencils}}} 
   %H1\tablefootnote{\label{fpdlabel}These benchmarks were ported from ~\cite{fpd}} & 392K & NA & NA & 2.22e-14 & 2108 / 274 s & 2.22e-14 & 4192 / 692 s & 2.22e-14 & 10579 / 2615 s \\
   H1\tnote{a} & 393K & NA & NA & \tb{1.11e-14} & \tb{1322} / \tb{274} & \tb{1.11e-14} & \tb{3767} / 692 & \tb{1.11e-14} & 10579 / 2615 \\
   H2\tnote{a} & 393K & NA & NA & \tb{1.94e-14} & \tb{1340} / \tb{275} & \tb{1.94e-14} & \tb{3792} / 694 & \tb{1.94e-14} & 10480 / 2603 \\
   H0\tnote{a} & 393K & NA & NA & \tb{5.55e-14} & 1334 / 280 & \tb{5.55e-14} & 3784 / 697 & \tb{5.55e-14} & 10472 / 2597 \\
   P1\tnote{a} & 436k & NA & NA & \tb{2.26e-14} & \tb{680} / 234  & \tb{2.26e-14} & \tb{1216} / \tb{360} & \tb{2.26e-14} &  2445 / 966  \\
   P2\tnote{a} & 436k & NA & NA & \tb{2.26e-14} & \tb{612} / 161 & \tb{2.26e-14} & \tb{1213} / 456 & \tb{2.26e-14} &  2428 / 942  \\
   P0\tnote{a} & 436k & NA & NA & \tb{7.55e-14} & 606 / 180  & \tb{7.55e-14} & 1225 / 458  & \tb{7.55e-14} & 2435 / \tb{998} \\
   C1\tnote{a} & 436k & NA & NA & \tb{6.25e-15} & \tb{1772} / 1186 & \tb{6.25e-15} & \tb{4122} / 3038 & \tb{6.25e-15} & 10875 / 7969 \\
   C2\tnote{a} & 436k & NA & NA & \tb{6.25e-15} & \tb{1170} / 1277 & \tb{6.25e-15} & \tb{4117} / \tb{2963} & \tb{6.25e-15} & 10766 / \tb{7980} \\
   C0\tnote{a} & 436k & NA & NA & \tb{5.56e-14} & 1593 / 914  & \tb{5.56e-14} & 4164 / 2827 & \tb{5.56e-14} & 10839 / 7946 \\
   Advection & 453k & \tb{1.01e-13} & \tb{3212 / 1479} & \tb{1.01e-13} & \tb{3218 / 1476} & \tb{1.01e-13} & \tb{3247 / 1623} & \tb{1.01e-13} & \tb{3215 / 1476} \\
   FDTD & 192k & \tb{3.71e-13} & %2.5 hrs & -- & -- & -- & -- & -- & -- \\
                             \tb{8902} & -- & -- & -- & -- & -- & --  \\
  %Stencils & H1 & 393K & NA & NA & 2.22e-14 & 2108 s & 2.22e-14 & 4192 s & 2.22e-14 & 10579 s \\
  %\midrule
  matmul-64x64 & 520K & \tb{4.76e-13} & 65 & \tb{4.76e-13} & 58 & \tb{4.76e-13} & 55 & \tb{4.76e-13} & 54 \\
  matmul-128x128 & 4177K & \tb{1.86e-12} & \tb{763} & \tb{1.86e-12} & \tb{664} & \tb{1.86e-12} & 556 & \tb{1.86e-12} & 527 \\
  %\midrule
  %{Tensor contraction} & 1530K & NA & NA & 4.55e-13 & 6309 & 4.55e-13 & 55902 & 4.55e-13 & 59640 \\
  %{Tensor contraction} & 1530K & NA & NA & \tb{2.28e-13} & 6309 & \tb{2.28e-13} & 55902 & \tb{2.28e-13} & 59640 \\
  {Tensor contraction} & 1530K & NA & NA & \tb{2.28e-13} & \tb{3676} & \tb{2.28e-13} & \tb{3115} & \tb{2.28e-13} & \tb{3142} \\
  {Tensor contraction}\tnote{b} & 1530K & NA & NA & 1.57e-19 & 1473 & 1.57e-19 & 953 & 1.57e-19 & 752 \\
  %\midrule
  %{Tref} & 22K & 1.16e-14 & 3 s & 1.55e-09 & 60 s & 3.38e-10 & 57 s & 1.25e-09 & 32 s \\
  {CG-Arc}\tnote{b} & 211K & \tb{3.15e-19} & \tb{1206} & 1.23e-17 & 2291 & 1.68e-17 & 1032 & 1.54e-17 & 3866  \\
  {CG-Pores}\tnote{b} & 45K & \tb{2.67e-05} & 9 & -- & -- & -- & -- & -- & -- \\
  %\midrule
  {Mol-Dyn}\tnote{c} & 5K & NA & NA & \tb{3.96e-14} & \tb{49} & \tb{4.46e-14} & \tb{117} & \tb{4.46e-14} & \tb{117} \\
  \tb{Serial Sum} & \tb{1023} & \tb{2.91e-11} & \tb{5407} & \tb{2.91e-11} & \tb{14} & \tb{2.91e-11} & \tb{11} & \tb{2.91e-11} & \tb{11} \\
  \tb{Reduction} & \tb{1023} & \tb{5.68e-13} & \tb{32} & \tb{5.68e-13} & \tb{34} & \tb{5.68e-13} & \tb{34} & \tb{5.68e-13} & \tb{34} \\
  \tb{Poly-50}   & \tb{1325} & \tb{3.26e-13} & \tb{3} & \tb{6.48e-13} & \tb{2} & \tb{6.25e-13} & \tb{2} & \tb{6.22e-13} & \tb{1.5} \\
  \tb{Horner-50} & \tb{100} & \tb{1.03e-13} & \tb{5} & \tb{4.43e-13} & \tb{2.6} & \tb{2.14e-13} & \tb{1.2} & \tb{2.58e-13} & \tb{1.3} \\
	\end{tabular}
	\begin{tablenotes}
	\item[a] Benchmarks ported from 
    % ~\cite{fpd} and ~\cite{10.1145/3402451}
	\item[b] Benchmarks analyzed over degenerate intervals
	\item[c] Benchmark realized from 
    % ~\cite{MD}
	\end{tablenotes}
	\caption{\label{tab:satire-results} Satire evaluated worst case absolute error bounds and execution time on larger benchmarks. }
 \end{threeparttable}
 \end{table*}
\endgroup


\noindent {\bf Larger Benchmarks:\/} Our larger
benchmarks cover stencils
(e.g., Finite-Difference Time-Domain FDTD), 
iterative solvers,
Fast Fourier Transforms (FFT),
Tensor Contractions, 
matrix multiplication
and Lorenz system of equations (a well-known nonlinear benchmark
that exhibits the
''butterfly effect'').
%
We ported the stencil kernels for heat (H*),
Poisson (P*) and Convection Diffusion (C) type  from
% ~\cite{fpd} 
and unrolled
them over 32 steps to be in \satire's input format.
%
The data range values for these 
variables were obtained by
scanning the input domain of their initial conditions.

For Conjugate Gradient solvers,
the input matrices were obtained from
% ~\cite{ufl}
and analyzed over 20 iterations of the solver. 
%
Tensor contractions are extensively used in computational chemistry codes.
%
We obtained smaller block level data for 4D tensor contractions from a
CCSD
% ~\cite{tensor} 
calculation on Uracil molecule, with the inner dimension of 35x35 for the
contraction.
%
For correctness of the contraction, the inner dimension is required
to be preserved, while the outer dimensions can be divided into
smaller partitions
for simplifying the problem. 

Table~\ref{tab:satire-results} summarizes the aforesaid large benchmarks
where column Direct Solve
indicates the bounds obtained without any abstractions. 
%
The ``Num OPs'' column shows the number of operators
in a single expression tree created by unrolling the loops
in these benchmarks to various sizes.
%
The unroll factors were chosen with two objectives:
(1)~push \satire to its limits, and (2)~mimic what a user
of \satire might do in the field to understand error-buildup
across iterations.
%
We neither attempt to compute a tight loop invariant nor determine
the fixed-point semantics of loops: these are known to be very difficult
for floating-point computations (see discussions in \S\ref{sec:relwork}).

For our linear benchmarks, path strength expressions aggregate to
constant factors, allowing huge scalability without abstractions.
%
For instance, {\em Direct Solve}
handles FDTD with $\approx 192K$ operators.
%
However for Lorenz, the path strength expressions are
quite complex symbolic expressions, and therefore abstractions were
essential at around 300 operators.
%
%Other nonlinear benchmarks
%(e.g., stencil applications and tensor contractions) also
%needed abstractions.




\noindent {\bf Abstractions:\/}  In our experiments pertaining
to abstraction, we did observe the competing forces
(e.g., the effects of frequent and infrequent abstractions)
mentioned in \S\ref{sec:abstractions} at play.
%
An encouraging observation was that
frequent abstractions did weaken the error bounds, but
by not much---they remain in the same order of magnitude.
%
Certain examples did suffer a lot:
in FDTD for example, concretization of internal nodes during
abstraction introduced larger correlation losses.
%
Fortunately, FDTD also does not critically depend on abstractions.
%
For such examples, correlations outweigh the need to abstract,
resulting in favorable error cancellations.

We chose three candidate abstraction windows in our experiments --- (10,20), (15,25) and (20,40).
In a majority of the cases, smaller abstraction
windows tended to estimate reasonably tight error bounds
while reducing the execution time dramatically.
%
This is especially impactful when many optimizer queries
are involved.
%
In the CCSD benchmark, \satire makes 26K and 12K optimizer queries for abstraction windows of
[10,20] and [20,40] respectively.
%
Although, the number of queries get halved, each query takes longer,  increasing
the total execution time -- {\em while in the end obtaining the same error bound.}

%% Sensitivity to code form changes
\begingroup
%\color{blue}
We now briefly discuss whether and how
semantics-preserving changes to one's code might impact abstraction.
%
Given that such changes modify the expression DAG,
round-off error bounds will also get affected correspondingly.
%
In one simple study, a 1,024 point serial
summation yielded an error bound of 2.91e-11
while a reduction-tree based summation of the
same items yielded an error bound of 5.68e-13
which is two orders of magnitude tighter.
%
In another simple study, we also compared
a straightforward polynomial calculation against
the Horner's method.
%
Both Horner's method and tree reduction
are known to be precision-preserving by design
than their counterparts (standard polynomial evaluations and
serial summation, respectively) as was confirmed by \satire.
%
We also observed that for the reduction scheme,
there is negligible impact due to abstraction.
%
For Horner's method,
we observe slight loss of tightness where the error bound drops from
the original bound of 1.0e-13 (without abstraction)
to 4.43e-13 when using an abstraction window of (10,20).
%
In summary, these equivalence-preserving transformations appear to
have the same order of magnitude of impact on the computed
error bounds either with or without abstraction.
%However, with larger abstraction depths the bound gets
%tighter as one would expect.
\endgroup


\noindent {\bf Result Reuse through Expression Hashing:\/ }
We now describe a result-reuse method that saves on computations.
%
Given that \satire abstracts all nodes at a selected height,
for time iterative kernels such as stencils, 
this boils down to abstracting all nodes in the plane of the selected intermediate tile,
which can be expensive in number of optimizer calls for a large tile size.
%
However, if the analysis of such kernels is done over input ranges that are
shared by multiple input variables,
many of these optimizer calls will result in
the same interval optimization query.
%
This can be taken advantage of
through a result-reuse method
implemented through a dictionary
that stores a compressed `md5' signature
of the query for each 
optimizer call as the key, and the previously
computed result as the value.
%
If two calls result in the same signature
(modulo variable re-namings),
the optimizer is bypassed and stored results are 
returned.
%
For the stencil types with
names H, P, C, and Advection,
we report two execution times for each configuration
where the numbers after
the ``/''
indicate the execution time with this option enabled.

\noindent{\bf Degenerate intervals :\/}
\satire supports the ability to feed degenerate input intervals
($[m,M]$ with $m=M$) to serve three purposes all of which
help improve analysis speed and/or versatility.
First, this allows to propagate sparsity information
by propagating 0s directly instead of interval ranges when
dealing with near-sparse matrices. This greatly simplifies the 
analysis since the corresponding symbolic variables are replaced using
constant propagation. 
%
The conjugate gradient (CG) benchmarks were executed on degenerate intervals
from two sparse matrices -- a computational fluid dynamics problem (Pores)
and a materials problem (ARC130). 
%

Next, it can help facilitate analysis when 
one encounters non-differentiable points (e.g., $E_1/E_2$ where
$E_2$'s interval includes $0$). Given that there is no direct way to circumvent
this problem, the provision for degenerate intervals allows 
the designer to architect selected points carefully to bypass the
discontinuities. In CG, when analyzed with interval ranges, beyond two iterations,
the scale factor, $\beta$, composed of the ratio of near zero residuals (from two successive iterations)
encounters a zero crossing interval in the denominator reporting a divide by zero error -- using degenerate
intervals remove these difficulties when such situations arise.
%

Additionally, this facility of degenerate intervals also
came in handy 
when studying the highly unstable Lorenz iteration scheme
where we could clamp a few inputs at degenerate values and explore
the remaining inputs (sensitivity analysis) across a non-degenerate interval.


\noindent {\bf Empirical consistency :\/}
We resort to extensive empirical testing to quantify the tightness and the empirical soundness of
\satire's worst case absolute error bounds.
%
We performed $10^6$ tests across these benchmarks (except the ones subject
to degenerate intervals)
%
with random sampling over their respective input intervals.
\satire's bounds were always
found to be conservative while being on average no worse that 2 orders of magnitude.
%
The stencil benchmarks obtain
a much tighter empirical
bound in the order of e-15.
%
Prefix-sum (Scan) obtained empirical bounds only one order of magnitude tighter
than the worst case bounds.
%
The largest deviation was seen of lorenz70, where \satire's
bound of \tb{1.06e-12} was two orders of magnitude
worse than empirically obtained maximum error of 4.1e-14.

\input{Evaluation/SC20-files/fft}

\input{Evaluation/SC20-files/lorenz}

\paragraph{Application to Relative error profiling}
\input{Evaluation/SC20-files/rel-error}

==> Evaluation/SC20-files/fft.tex <==

\paragraph{\textbf{FFT: A Case study} } Fast Fourier transform (FFT) is an optimized algorithm for
discrete Fourier transform (DFT), which converts a finite sequence of sampled points
of a function into a same length sequence of an equally numbered complex-valued
frequency components.
%
It has a vast number of applications in signal processing and
fast multi-precision arithmetic for large polynomial and integer multiplications.
%
\label{page:fft}

An $N$-point FFT involves $\log_2N$ stages, each stage having a familiar butterfly structure
(see for example
% ~\cite{hal-fft}
).
%
We are not aware of any tool supporting floating-point error analysis over complex domains
barring
% ~\cite{boland} 
which was demonstrated on a small 64-point FFT design.
%except in~\cite{boland} that performed analysis for a small 64 point FFT.
%
However, its application to fast math multi-precision libraries necessitates 
precise floating point error analysis and has been the subject of multiple
analytical studies
% ~\cite{ramos,percival-mult,percival-fft,schwarzlander-fft}.
%
These analysis methods focus on
obtaining L2-norms in terms of root mean square (RMS) errors, or statistically profiled
error bounds.
%
Brisbarre et al.
% ~\cite{hal-fft} 
followed up on the work from Percival's
% ~\cite{percival-fft,percival-mult}
to report the best L2-norm bound till date of $\approx 30.99 ulps$.
%
That is, if $z$ represents the
discretized input samples, $Z$ is the exact result and $\hat{Z}$ is the computed result, 
then,
%\begin{equation}
%\label{eq:fft-l2}
 $  \dfrac{||Z - \hat{Z}||_2}{||Z||_2} \leq B \approx 30.99 {\bf u} $
%\end{equation}

To extend this result to a bound on absolute error corresponding to the
L-infinity norm,
we utilize two well-known relations: (1)~Between the L2 norms of the
input and outputs of an $N$-point FFT, i.e., $||Z||_2 \leq \sqrt{N} \cdot ||z||_2$,
and (2)~a generic relation between the L-infinity norm and L2-norm, i.e., 
$||Z||_2 \leq \sqrt{n}||Z||_\infty$.
%
Using these relations, the L-infinity norm on the
error (as obtained in
% ~\cite{hal-fft}) 
of the computed FFT result can be obtained as \\[-1em]
\begingroup
\small
\begin{equation}
\label{eq:fft-inf}
\begin{split}
  ||Z - \hat{Z}||_\infty \leq B\cdot N \sqrt{2} ||z||_\infty
\end{split}
\end{equation}
\endgroup
%\vspace*{-2.5ex}

Equation$~\eqref{eq:fft-inf}$ \tb{obtains} the absolute-error bound analytically.
%Using equation$~\eqref{eq:fft-inf}$ the absolute-error bound can be obtained analytically.
%
%Plugging in the best bound seen for l2-norm, $B$, in equation $~\eqref{eq:fft-inf}$
%obtains the corresponding the maximum absolute error bound analytically.
A 1024-point FFT with input  samples in the interval $[0,1]$ with
an L2-norm bound of $B \approx 30.99 {\bf u}$ obtains an absolute error bound of $78200 {\bf u}$.
%
For double precision data type, with ${\bf u} = 2^{-53}$, implying an absolute error bound of
\textbf{4.98e{-12}}.

\satire partitions the real and imaginary parts
of the complex operations in FFT,
obtaining real expression types for the 
output variables guarded with rounding information at every compute stage.
%
Two separate datapaths are generated for the 
real and imaginary terms, each of which is solved individually.
%
%It then solves each of them individually.
%
Let $E_R$ and $E_I$ denote the absolute error bounds obtained by solving
the real and imaginary parts, respectively.
%
These solutions, on their own, provide the individual accuracy information of the
real and imaginary expressions.
%
Additionally, $E_T = \sqrt{E_R^2 + E_I^2}$ gives the
bound on the maximum of the total absolute error.
%
It is an upper bound on the
L-infinity norm.

We show that \satire obtains a tighter bound than the analytical
bound obtained by
% ~\cite{hal-fft} 
as in Equation$~\eqref{eq:fft-inf}$.
%
We also select
the input space in the interval $[0,1]$.
%
The bound obtained for the real and imaginary parts are 
$E^R \leq \hbox{\tb{3.98e{-13}}}\ $ and $E^I \leq \hbox{\tb{3.80e{-13}}}$.
%
Thus the total error bound is 
$E_T \leq $ \tb{\textbf{5.5e{-13}}} which is tighter  than the best analytical bound obtained
in
% ~\cite{hal-fft}
. 
%
We tried different input intervals for FFT, each time obtaining a tight bound
in comparison to the analytical bounds achievable due to
% ~\cite{hal-fft}
. However, the optimizer
faced convergence difficulties for intervals with zero crossings like $[-1,1]$.
In these cases, incrementally solving using abstraction of smaller depths allowed
us to solve the problem while still obtaining tighter bounds than
% ~\cite{hal-fft}
.
%with rigorous information on the individual accuracies of the
%partitioned datapaths.



==> Evaluation/SC20-files/lorenz-table.tex <==
\begingroup
\small
\begin{table}[ht]
\centering
%\makebox[0pt][c]{\parbox{0.8\textwidth}{%
%\begin{minipage}[b]{0.5\hsize}
\begin{tabular}{ccccccc}
\toprule
\multirow{3}{*}{Lorenz} & \multicolumn{6}{c}{Window of Abstraction depth : (mindepth, maxdepth)} \\
\cmidrule(lr){2-7}
& \multicolumn{2}{c}{(10,20)} & \multicolumn{2}{c}{(15,25)} & \multicolumn{2}{c}{(20,40)} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
				 & err 		& \shortstack[1]{Exec \\Time}			 & err		& \shortstack[1]{Exec \\Time} 			& err 		& \shortstack[1]{Exec \\Time}  \\
lorenz20: x	 & \tb{5.69e-15} & \multirow{3}{*}{\tb{14s}}	 & \tb{5.88e-15} & \multirow{3}{*}{\tb{535s}} 	& \tb{5.64e-15}  & \multirow{3}{*}{\tb{545s}}  \\
lorenz20: y	 & \tb{1.25e-14}	&  		 				 & \tb{1.25e-14} &   		 				& \tb{1.24e-14}	& 	\\
lorenz20: z	 & \tb{4.75e-15}	&  		 				 & \tb{4.82e-15} &   		 				& \tb{4.72e-15}	& 	\\
\cmidrule(lr){2-7}
lorenz40: x	 & \tb{3.78e-14} & \multirow{3}{*}{29s}	 & \tb{3.91e-14}	& \multirow{3}{*}{1131s}	& \tb{3.75e-14}	& \multirow{3}{*}{1192s}	\\
lorenz40: y	 & \tb{9.11e-14} &     		 			 & \tb{9.33e-14}	&    		 				& \tb{9.02e-14}	& 	\\
lorenz40: z	 & \tb{7.08e-14} &     		 			 & \tb{7.09e-14}	&    		 				& \tb{6.95e-14}	& 	\\
\cmidrule(lr){2-7}
lorenz70: x	 & \tb{3.02e-13} & \multirow{3}{*}{\tb{50s}}	 & \tb{2.45e-13}	& \multirow{3}{*}{\tb{2088s}}	& \tb{2.45e-13}	& \multirow{3}{*}{\tb{2150s}}	\\
lorenz70: y	 & \tb{1.06e-12} &     		 			 & \tb{7.93e-13}	&    		 				& \tb{7.93e-13}	& 	\\
lorenz70: z	 & \tb{1.05e-12} &     		 			 & \tb{8.14e-13}	&    		 				& \tb{8.14e-13}	& 	\\
\end{tabular}
\caption{Error bounds for the three state variables in the Lorenz equation}
\label{tab:lorenz-table}
%\end{minipage}
%}
%}
\end{table}
\endgroup


==> Evaluation/SC20-files/lorenz.tex <==
%\vspace*{1em}
\paragraph{{\textbf{Lorenz equations: A Case Study}}}
\label{para:lorenz}
%
Lorenz equations model thermally induced fluid convection
using three state variables $(x,y,z)$.
%
Here, $x$ represents the fluid velocity amplitude,
$y$ models temperature difference between top and bottom membranes,
while $z$ represents a distortion from linearity of temperature
% ~\cite{lorentz}
.
%
The equation requires three additional parameters, $a$=10 called the Prandtl number,
$b$=8/3 corresponding to the wave number for the convection, and
$r$ being the Rayleigh number proportional to the
temperature difference. 
%
The recurrence relations obtained by discretizing the continuous 
version of the Lorenz equation are shown in Equation$~\eqref{eq:lorenz-discrete}$,
where $k$ represents the previous iteration and $dt$ is the time discretization. 
%\vspace*{-0.5ex}
\begingroup
\small
\begin{equation}
\label{eq:lorenz-discrete}
 \begin{split}
 	x_{k+1} &= x_k + a(x_k - y_k)dt \\
	y_{k+1} &= y_k + (-x_kz_k + rx_k - y_k)dt \\
	%y_{k+1} &= y_k + (-x_kz_k + rx_k - y_k)dt \\
	z_{k+1} &= z_k + (x_ky_k - bz_k)dt \\
 \end{split}
\end{equation}
\endgroup
In
% ~\cite{lorentz}
, authors study the trajectories for different $r$ values 
for chosen initial conditions of $(x_1,y_1,z_1,dt)=(1.2,1.3,1.6,0.005)$.
%
It shows chaotic behavior for $r \geq 22.35$ and again starts approaching equilibrium once $r$
reaches close to 200.
%
However, for such chaotic systems, if two initial conditions differ by 
a quantity of $\delta$, the resulting difference after time $t$ shows exponential
separation in terms of $\delta \cdot e^{\lambda t}$.
%
This becomes a critical component when
evaluating such equations in finite precision since the round-off error accumulation
introduces a gradual $\delta$ error building up.

%The floating-point error accumulated introduces a proxy for the $\delta$ error build up,
%also introducing exponential separation.
%between the actual and computed trajectories.
%Obtaining precise error bounds for such computations thus becomes important. 
%
We focus on two aspects of the analysis: (1)~Obtaining bounds over a range
of input intervals over $(x,y,z)$,
%thus obtaining bounds for a known range
%of initial conditions
and (2)~Analyze the sensitivity of initial conditions on individual
inputs by using degenerate intervals on the other inputs.
%
%Such analysis is essential for
%nonlinear chaotic systems which can become unstable from accumulated noise due to 
%`exponential separation'.

%Beyond a few iterations, the non-linearity involved in these equations
%impede the application of current tools such as FPTaylor.
%
%Using FPTaylor, it took 350 seconds to generate Taylor forms for a small 5-iteration case,
%while timing out for unrolls beyond 10 iterations.
%FPTaylor took around 350 seconds to build the taylor forms for an unroll of 5 iterations
%while timing out beyond an hour for 10 iterations.
%
%Additionally, the symbolic Taylor
%form for 5 iterations was so large that backend optimizer could not handle.


%
%In this analysis we discuss how abstraction allows us to push the
%limits of analysis significantly while also highlighting when it hits certain limits.
%beyond which it looses significance.

Using \satire{}, we obtain tight bounds for as large as 70 iterations of the problem using
abstractions.
%
Note here the non-linearity of
these equations makes it difficult to simplify expressions beyond a certain limit.
%
The error expressions composed of the products of forward error and reverse derivative
may reach a large operator count quickly within few iterations, choking {\tt symEngine}'s
simplification process.
%
\satire delays further canonicalization beyond an operational count larger than a pre-defined limit,
controlled by a parametric knob, $maxOpCount$, with default value of $30K$ selected 
over multiple experiments over a mix of non-linear and linear systems.
%
Using $maxOpCount$, we only allow simplification within the depth
necessary for abstraction or otherwise force abstraction at a reduced height.
During the next abstraction, further simplification take place.
%Over say 20 iterations, the completely flattened expression may reach an operation count of over 100K
%for the error expression which is a combination of the forward error and reverse derivatives. 
%%
%To reduce the overhead of SimEngine, we do not simplify the expression nodes beyond the 8K heuristically. 
%%

%\skcmtside{Don't quite get this sentence}
%Furthermore, we require abstraction guidance here else the large expression sizes will become untenable for the optimizers. 
%
%For example, for the Lorenz-20 (that is unrolled over 20 iterations), the overall AST depth is 90.
Table~\ref{tab:lorenz-table} shows the
bounds obtained for varying windows of the abstraction depth and
the corresponding execution time (exec time) in seconds.

\input{Evaluation/SC20-files/lorenz-table}
\vspace*{-1ex}
%\begingroup
%\small
%\begin{table*}[ht]
%\centering
%\makebox[0pt][c]{\parbox{0.8\textwidth}{%
%\begin{minipage}[b]{0.5\hsize}
%\begin{tabular}{ccccccc}
%\toprule
%\multirow{3}{*}{Lorenz} & \multicolumn{6}{c}{Window of Abstraction depth : (mindepth, maxdepth)} \\
%\cmidrule(lr){2-7}
%& \multicolumn{2}{c}{(10,20)} & \multicolumn{2}{c}{(15,25)} & \multicolumn{2}{c}{(20,40)} \\
%\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
%				 & err 		& exec\_time 			 & err		& exec\_time 			& err 		& exec\_time  \\
%lorenz20: x	 & 1.16e-14 & \multirow{3}{*}{12s}	 & 1.19e-14 & \multirow{3}{*}{519s} 	& 1.14e-14  & \multirow{3}{*}{528s}  \\
%lorenz20: y	 & 2.54e-14	&  		 				 & 2.54e-14	&   		 				& 2.52e-14	& 	\\
%lorenz20: z	 & 9.62e-15	&  		 				 & 9.84e-15 &   		 				& 9.64e-15	& 	\\
%\cmidrule(lr){2-7}
%lorenz40: x	 & 7.79e-14 & \multirow{3}{*}{29s}	 & 8.04e-14	& \multirow{3}{*}{1131s}	& 7.69e-14	& \multirow{3}{*}{1192s}	\\
%lorenz40: y	 & 1.93e-13 &     		 			 & 1.96e-13	&    		 				& 1.88e-13	& 	\\
%lorenz40: z	 & 1.49e-13 &     		 			 & 1.52e-13	&    		 				& 1.48e-13	& 	\\
%\cmidrule(lr){2-7}
%lorenz70: x	 & 1.64e-11 & \multirow{3}{*}{49s}	 & 9.18e-12	& \multirow{3}{*}{2050s}	& 9.18e-12	& \multirow{3}{*}{2079s}	\\
%lorenz70: y	 & 2.76e-10 &     		 			 & 1.06e-10	&    		 				& 1.06e-10	& 	\\
%lorenz70: z	 & 2.83e-10 &     		 			 & 1.14e-10	&    		 				& 1.14e-10	& 	\\
%\end{tabular}
%\caption{Error bounds for the three state variables in the Lorenz equation}
%\label{tab:lorenz-table}
%\end{minipage}
%}}
%\end{table*}
%\endgroup
%Table ~\ref{tab:lorenz-table} shows the execution time and error bounds obtained
%by \satire for three different levels of abstraction. 
We perform analysis for 20, 40, and
70 iterations. The second state variable, $y$, shows more worst-case variation. 
Therefore, we studied the sensitivity of $y$ for a larger size of 70 iterations 
using degenerate intervals in $x$ and $y$,
obtaining a bound of \tb{5.50e-13} as opposed to \tb{8.14e-13} in the non-degenerate case.


==> Evaluation/SC20-files/rel-error.tex <==
After having obtained the worst case absolute error for an
expression $g$ over input intervals $I$ using \satire, suppose the user
wants to run their code, say instantiated at double precision (dp),
with inputs $i$ chosen from $I$  and
wants to obtain the worst case
{\em relative error} estimates during that run.
%
This can be useful for the user, as relative error directly
($RE$) informs about {\em precision loss}.
%
$RE$ is defined by
$RE(g) = ({|g - \tilde{g}|}/{g})$ where the numerator is the
absolute error (``true-value - computed-value'')
and the denominator the ``true-value.''
%
The \satire-obtained worst-case absolute error over $I$
is an upper-bound for the numerator of $RE(g)$.
%
The ``true value'' (denominator) can be 
obtained by instrumenting the code in higher precision (say quad-precision)
and obtain $g_{qp}$ as a close proxy to $g$, allowing us
to compute an upper bound on $RE(g)$.
%
The user can then estimate the number of bits
lost as $\# bits\ lost = ceil(\log_2(RE(g)/{\bf u})$)
where $\bf{u}$ is the unit round-off.

Unfortunately, obtaining $g_{qp}$ in this manner calls for code-instrumentation.
%
Suppose we employ $g_{dp}$ in lieu of $g_{qp}$: how much error are we introducing
in our relative error estimation?
%
Since $g_{dp}$ is the observed value at runtime, there is no extra overhead to evaluate
this quantity (unlike shadow value calculations). 
%
To determine that, we first obtain an equation
characterizing
the discrepancy in lost-bits estimation, calling it $Q$: \\[-2em]

    \begin{equation}
		\label{eq:compare-rel-error}
	  \begin{split}
		Q &= q_{sat} - q_{shadow}; \; {\rm where} \\
		q_{sat} &=   log_2(\; \max(|g - \tilde{g}|) / (|g_{dp}|\cdot {\bf u}) ) \\
		q_{shadow} &= log_2(\; \max(|g_{qp} - g_{dp}|) / (|g_{qp}|\cdot {\bf u}) ) 
	  \end{split}
    \end{equation}
%

We now estimate the spread of $Q$ across multiple
simulation runs, each time starting the simulation
at an $i$ value drawn at random from within $I$.
%
For such simulations, if we plot $Q$, we are able to determine
the spread of
discrepancy in estimating the number of bits lost,
shown in Figure~\ref{fig:fdtd-rel-error}, where
y-axis plots the 
spread of $Q$,
and the x-axis plots the simulation runs
involved in generating those $Q$s.
%
For this method to be (empirically) sound, $Q$ must stay above zero.
%
In addition, if $Q$ stays close to $0$,
it would tend to confirm the tightness of the relative
error estimation.


\noindent{\em Observations about $Q$ in our Simulations:\/}
We do find that $Q > 0$, confirming that this relative
error estimation method is sound in an empirical sense.
%
In our studies,
we analyzed a subset of our benchmarks (H0, C0, P0, Prefix-sum, DQMOM, FDTD, FFT and lorenz20) 
as part of this case study.
%selected from stencils, DQMOM and FFT as part of this case study.
%
We chose $I=[0,1]$, thus ensuring that it contains many binades
of floating-point values (many exponent changes involved in the
range $[0,1]$).
%
This ensures that we pick values with widely differing
exponents as our candidate $i$, thus causing higher overall error.


\begin{figure}[t]
    \centering
    %\includegraphics[width=1.2\columnwidth,height=0.8\columnwidth]{figs/fdtd-rel-error.PNG}\\[-0.5em]
    \includegraphics[width=1\columnwidth,height=0.75\columnwidth]{Evaluation/SC20-figs/rel-error.pdf}\\[-0.5em]
    \caption{\label{fig:fdtd-rel-error}
x-axis: number of simulations performed for high precision shadow value evaluation;
y-axis: Measured $Q$}
\end{figure}




%\vspace{-0.5ex}
%\begin{figure}
%  \begin{minipage}{.25\textwidth}
%    %\begin{equation}
%	%	\label{eq:bits-lost}
%	%  \# bits\ lost = p - \log_2(re(f)/{\bf u})
%    %\end{equation}
%    \begin{equation}
%		\label{eq:compare-rel-error}
%	  \begin{split}
%		Q &= qsat - qshadow; \\
%		qsat &= \dfrac{\max(|f - \tilde{f}|)}{|f_{dp}|} ; \\
%		qshadow &= \dfrac{|f_{qp} - f_{dp}|}{|f_{qp}|}; \\
%	  \end{split}
%    \end{equation}
%  \end{minipage}\hfill
%  \begin{minipage}{.70\textwidth}
%    \centering
%    %\includegraphics[width=1.2\columnwidth,height=0.8\columnwidth]{figs/fdtd-rel-error.PNG}\\[-0.5em]
%    \includegraphics[width=0.8\columnwidth,height=0.6\columnwidth]{figs/rel-error.pdf}\\[-0.5em]
%    \caption{\label{fig:fdtd-rel-error}
%Difference in precision estimate(\# bits lost) between \satire and shadow value calculation}
%    \end{minipage}
%\end{figure}

% 
Figure~\ref{fig:fdtd-rel-error} plots the results of
our empirical evaluation 
for 10K simulations of this subset of benchmarks.
%
We observe that
for well-conditioned 
problems presented in the upper half of Figure~\ref{fig:fdtd-rel-error} 
(smoothing solvers such as 2-D heat---H0 in our figure),
the prediction difference lies in the range of 6 to 8 bits---a good
confirmation of the tightness of our estimation method.
%
For more complex computations presented in the lower half of
the figure
(e.g.,  DQMOM, FFT, etc), the spread of $Q$ is higher.
%
Yet, we do see many $Q$ values bunched up within tight bands.
%
The lower bound of these bands indicate the extent
of tightness exhibited by our relative error profiling method
(this despite our use of \satire's worst-case bounds in the numerator
of $q_{sat}$).


In conclusion, the approach presented offers a promising 
avenue for estimating precision loss---at least in a relative sense---through
the following simple steps: (1)~measure the worst-case absolute error,
(2)~observe the runtime output value of the function being studied, and
(3)~apply the formula for $q_{sat}$.
%
Armed with this knowledge of precision loss, a user may be able to
profile their simulation to identify points at which
it exhibits high relative error
(e.g., as a result of the value distribution that exists at those
simulation states) and mitigate the precision loss suitably---say
by rewriting their function, switching to higher precision
realizations, etc.



%--end


%--




==> Evaluation/STATIC25-eval.tex <==
\section{Random-testing Results}

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.43]{Evaluation/STATIC25-figs/Varity_results.png}
    \caption{Analysis Results for 1000 Varity-generated Random Floating-Point Programs}
    \label{fig:1000tests}
\end{figure}

We discovered that \satirenospace's crashes are {\em often} due to the fact that the symbolic error expressions generated contained sub-expressions of the form $a/b$ where the interval for $b$ could include zero (see Section~\ref{non-robustness_of_error_analyzers}), thus causing $a/b$ to evaluate to infinity.

For \varity, we arbitrarily set the input intervals of each scalar input variable as $[-1,1]$ which is fairly aggressive, and often the default choice for an ``acid test.''\footnote{Half the representable floating-point numbers are in this range, and also this interval includes $0$ which often leads to exceptions and unwanted/unexpected results.} and double precision type. We restricted the generated programs to about 
40-operator expressions (a number picked to be able to quickly run through 1,000 random programs).

We observed (Figure \ref{fig:1000tests} please focus on the green \seesawg bars first; the ``G'' suffix stands for \satire with the \gelpia
% ~\cite{gelpia-github} 
optimizer) that \seesawg crashes for $\approx$ 32\% of programs, results in a useful error bound in  $\approx$ 20\% of programs, and for $\approx$ 48\% of programs results in an infinity error bound.
%
The reason for infinity error bound is the error expression containing sub-expressions that optimize to infinity for some part of the input domain. 
%
As described earlier, some of these domain points are avoided in \fpguard using a combination of error intervals and constraint synthesis.

After incorporating the \ibex solver in lieu of \gelpiaspace in
 \seesawi (Figure~\ref{fig:1000tests}; please focus on the blue \seesawi bars, where  ``I''  stands for \ibexnospace), we observed a distinct improvement: the number of programs that crashed decreased from 321 to 133 programs with respect to \seesawg, which means that $\approx$ 87\% of programs passed in comparison to $\approx$ 68\% before. This lead to a slight increase in the number of reasonable answers but a larger increase in infinity cases, reflecting the known weakness of  using randomly generated programs using the interval $[-1,1]$.
Finally, \fpguard  where we handled division by zeros, increased  the number of reasonable error bounds by $\approx$ 18\%, which correspondingly also reduced the number of infinity cases by 177. The remaining causes of infinity can be reasonably attributed to other functions that characteristically that lead to singularities. These trends do translate to an improvement over realistic case studies, discussed next.

\section{Realistic case studies}

\textbf{Experimental Setup:} We ran \satire versions using Python-3.9 on a dual 4-core Intel i5-8279U 2.40GHz CPU (total 8 cores) with 16GB of RAM. Although \seesawg supports multi-core parallelism, this evaluation does not invoke this feature to allow more direct comparisons with previous \seesawg evaluations conducted in 
% \cite{2021_Das}
.

\subsection{Domain-Constraints Study}
\input{Evaluation/STATIC25-files/domain-constraints}
\input{Evaluation/STATIC25-files/table-constraints}

\subsection{Solver Study} \label{solver study}
\input{Evaluation/STATIC25-files/solver_study}
\input{Evaluation/STATIC25-files/gelpia_vs_ibex}
\input{Evaluation/STATIC25-files/table_idc}



==> Evaluation/STATIC25-files/domain-constraints.tex <==
Among the existing \satire benchmarks, 
we discovered
that
two benchmarks
(namely DistSinusoid and SmartRoot)
produce infinity as the
absolute error estimate,
while one benchmark 
(namely Test2) produces infinity after 
only a 
small increase in the input domain (hence merits, for robustness sake, an input domain
correction).
%
For these benchmarks,
we proceed to apply constraints generated by the combination of error intervals and constraint synthesis.
%
Table~\ref{tab:constraint-inference} presents
the obtained domain constraints to avoid infinity. We get constraints corresponding to four singular points for  DistSinusoid, two for Test2 and one for SmartRoot.
%

==> Evaluation/STATIC25-files/gelpia_vs_ibex.tex <==
\begin{table}[ht]
    \centering
    
    \begin{tabular}{lrrrr}
    \toprule
         \multirow{2}{*}{Benchmark} & \multicolumn{2}{c}{Absolute Error} & \multicolumn{2}{c}{Execution Time (sec)} \\
         \cmidrule(lr){2-3} \cmidrule(lr){4-5}
          & \seesawgnospace & \seesawinospace & \seesawgnospace & \seesawinospace \\
    \hline
    \midrule
        Barycentric & - & 3.01e-15 & - & 494.38 \\
        SymSchur & 4.23e-16 & \textbf{4.05e-16} & 69.71 & \textbf{2.70} \\
        SquareRoot3 & \textbf{5.52e-16} & 5.53e-16 & 2.29 & \textbf{0.12} \\
        DistSinusoid & inf & inf & 61.10 & \textbf{19.11} \\
        Lin Interpolator & 1.47e-14 & 1.47e-14 & 2.18 & \textbf{0.37} \\
        Non-lin Interpola & 4.44e-16 & \textbf{4.43e-16} & 22.14 & \textbf{0.20} \\
        Enclosing Sphere & 4.64e-15 & \textbf{4.38e-15} & 75.14 & \textbf{20.53} \\
        Cubic Spline & \textbf{4.15e-16} & 4.16e-16 & 25.66 & \textbf{0.87} \\
        Gram-Schmidt & 1.28e-16 & \textbf{1.19e-16} & 731.62 & \textbf{305.98} \\
        Poisson & 1.00e-17 & 1.00e-17 & 2117 & \textbf{19.24} \\
        Closest Point & 3.40e-15 & \textbf{1.55e-15} & 152.47 & \textbf{31.57} \\
        Test2 & 1.34e-13 & \textbf{5.54e-14} & 231.33 & \textbf{1.11} \\
        Styblinski & \textbf{1.40e-14} & 1.41e-14 & 49.17 & \textbf{1.31} \\
        Sphere Point & - & 5.12e-15 & - & \textbf{470.74} \\
        Lead-Lag & 9.98e-18 & 9.98e-18 & 142.97 & \textbf{4.35} \\
        Eigensphere & - & 1.30e-15 & - & \textbf{756.11} \\
        Jacobi & 4.32e-13 & \textbf{3.56e-13} & 185.47 & \textbf{43.87} \\
        Mol-Dyn & 2.94e-15 & 2.94e-15 & 274.23 & \textbf{21.19} \\
        SmartRoot & inf & inf & 46.89 & \textbf{0.94} \\
    \bottomrule
    \end{tabular}
    \vspace*{2mm}
    \caption{Comparison of \satire with \gelpia as a global optimizer vs \satire with \ibex as a global optimizer}
    \label{tab:solver-comparison}
\end{table}

==> Evaluation/STATIC25-files/solver_study.tex <==
Table~\ref{tab:solver-comparison} presents the absolute error estimates and execution
time on the benchmarks in \seesawg and \seesawinospace.
%
Across all benchmarks, \seesawi has proven to
be faster at estimating
the worst-case error than \seesawgnospace.
%
In most cases \seesawi
reports a tighter error bound than \seesawg.
%
Also, in all
cases the error bound reported by both versions is in the same
order of magnitude.
%
The performance of \seesawi is strictly better in all cases.
%
Since the main change 
going from
 \seesawg to \seesawi is a global optimizer replacement, 
 our conclusion is
 that
 \ibex  is a better optimizer to employ than
 \gelpia from the point of view
  of floating-point
  error analysis.

Table~\ref{tab:preconditioned-errors} presents the absolute error estimates 
along with execution times of \seesawi and \fpguard on the three benchmarks in Table~\ref{tab:constraint-inference} for which \satire provided an unusable analysis.

In summary,
our evaluation empirically supports the possibility that our techniques developed based purely on random testing tend to benefit realistic benchmarks as well.
%
More remarks on random testing
are presented in Section~\ref{sec:conc}.




==> Evaluation/STATIC25-files/table-constraints.tex <==
\begin{table}[ht]
    \centering
    
    \begin{tabular}{lp{6cm}}
    \toprule
         Benchmark & Constraints \\
    \hline
    \midrule
       DistSinusoid &  $[k2 - k1 + 1.75193839388411 + \epsilon \leq 0  \mid -1.0 * (k2 - k1 + 1.75193839388411) + \epsilon \leq 0]$ \textbf{\&} \\ &
	 $[k2 - 1.0 + \epsilon \leq 0  \mid -1.0 * (k2 - 1.0) + \epsilon \leq 0]$ \textbf{\&} \\ & $[k1 + \epsilon \leq 0  \mid -1.0 * k1 + \epsilon \leq 0]$ \textbf{\&} \\ &	$[k1 - (k2 + 1.75193839388411) + \epsilon \leq 0  \mid -1.0 * (k1 - (k2 + 1.75193839388411)) + \epsilon \leq 0]$ \\
        \midrule
        Test2 & $[x1 + \epsilon \leq 0  \mid -1.0 * x1 + \epsilon \leq 0]$ \textbf{\&} \\ &
	 $[x2 + 1.0 + \epsilon \leq 0  \mid -1.0 * (x2 + 1.0) + \epsilon \leq 0]$ \\
        \midrule
        SmartRoot & $[	 (c - 1.02083333333333 + \epsilon \leq 0)  \mid (-1.0 * (c - 1.02083333333333) + \epsilon \leq 0)]$
\\
    \bottomrule
    \end{tabular}
    \vspace*{2mm}
    \caption{Constraints inferred from \fpguard generated error expressions. The $\epsilon$ variable is a user-provided ``knob'' that can allow more of the domain to be avoided based on its value}
    \label{tab:constraint-inference}
\end{table}

==> Evaluation/STATIC25-files/table_idc.tex <==
\begin{table}[ht]
    \centering
    
    \begin{tabular}{lrrrr}
    \toprule
         \multirow{2}{*}{Benchmark} & \multicolumn{2}{c}{\shortstack[l]{Absolute \\Error}} & \multicolumn{2}{c}{\shortstack[l]{Execution\\ Time (sec)}} \\
         \cmidrule(lr){2-3} \cmidrule(lr){4-5}
          & \seesawinospace & \fpguard & \seesawinospace & \fpguard\\
    \hline
    \midrule
        DistSinusoid & inf & 1.70e-15 & 19.11 & 43.57\\
        Test2 (modified) & inf & 1.77e-14 & 17.41 & 8.86 \\
        SmartRoot & inf & 1.26e-15 & 0.94 & 1.09 \\ 
    \bottomrule
    \end{tabular}
    \vspace*{2mm}
    \caption{Comparison of \seesawi vs \fpguard for the Cases Where Infinity is the Worst-Case Absolute Round-off Error by Default}
    \label{tab:preconditioned-errors}
\end{table}

==> Evaluation/TACO25-files/lorenz.tex <==
%\vspace*{1em}
% \paragraph{{\textbf{Lorenz equations: A Case Study}}}
\subsubsection{\textbf{Lorenz equations: A Case Study}}
\label{para:lorenz}
%
The Lorenz equations model thermally induced fluid convection using three state variables $(x,y,z)$.
Here, $x$ represents the amplitude of fluid velocity, $y$ corresponds to the temperature difference between the top and bottom membranes, and $z$ signifies a deviation from the linear temperature profile~\cite{lorentz}.
%
The equations require three additional parameters: $a=10$, known as the Prandtl number; $b=8/3$, representing the wave number for convection; and $r$, the Rayleigh number, which is proportional to the temperature difference. 
%
The recurrence relations obtained by discretizing the continuous Lorenz equations are shown in Equation~\eqref{eq:lorenz-discrete}. Here, $k$ represents the previous iteration, and $dt$ denotes the time step used for discretization.


%\vspace*{-0.5ex}
\begingroup
\small
\begin{equation}
\label{eq:lorenz-discrete}
 \begin{split}
 	x_{k+1} &= x_k + a(x_k - y_k)dt \\
	y_{k+1} &= y_k + (-x_kz_k + rx_k - y_k)dt \\
	%y_{k+1} &= y_k + (-x_kz_k + rx_k - y_k)dt \\
	z_{k+1} &= z_k + (x_ky_k - bz_k)dt \\
 \end{split}
\end{equation}
\endgroup

In~\cite{lorentz}, the authors investigate the system's trajectories for various values of $r$, starting from the initial conditions $(x_1,y_1,z_1,dt)=(1.2,1.3,1.6,0.005)$. The results reveal chaotic behavior for $r \geq 22.35$, while the system begins to approach equilibrium as $r$ approaches 200.

For chaotic systems, a small difference $\delta$ in initial conditions leads to an exponential divergence over time, described by $\delta \cdot e^{\lambda t}$. This exponential separation plays a significant role in numerical evaluation, as the accumulation of round-off errors introduces a gradually increasing $\delta$.
Our analysis focuses on two key aspects:
\begin{enumerate}
    \item Obtaining bounds over a range of input intervals for $(x,y,z)$.
    \item Analyzing the sensitivity of initial conditions by using degenerate intervals for some inputs while varying others.
\end{enumerate}
    
%Such analysis is essential for
%nonlinear chaotic systems which can become unstable from accumulated noise due to 
%`exponential separation'.

%Beyond a few iterations, the non-linearity involved in these equations
%impede the application of current tools such as FPTaylor.
%
%Using FPTaylor, it took 350 seconds to generate Taylor forms for a small 5-iteration case,
%while timing out for unrolls beyond 10 iterations.
%FPTaylor took around 350 seconds to build the taylor forms for an unroll of 5 iterations
%while timing out beyond an hour for 10 iterations.
%
%Additionally, the symbolic Taylor
%form for 5 iterations was so large that backend optimizer could not handle.


%
%In this analysis we discuss how abstraction allows us to push the
%limits of analysis significantly while also highlighting when it hits certain limits.
%beyond which it looses significance.
Using \satire, we obtain tight bounds for up to 70 iterations of the problem through the use of abstractions.
Notably, the non-linearity of these equations poses significant challenges for simplifying expressions beyond a certain limit.

The error expressions, which consist of products of forward errors and reverse derivatives, can quickly grow in operator count after only a few iterations. This often overwhelms {\tt symEngine}'s simplification process.

To address this, \satire delays further canonicalization when the operator count exceeds a predefined limit, controlled by the parameter $maxOpCount$. The default value of $maxOpCount$ is set to 30,000, determined through extensive experimentation across a mix of non-linear and linear systems.

By leveraging $maxOpCount$, simplifications are restricted to the depth necessary for abstraction. When the operator count exceeds this limit, abstraction is enforced at a reduced height. Subsequent abstractions then allow for further simplifications.

Table~\ref{tab:lorenz-table} shows the
bounds obtained for varying windows of the abstraction depth and
the corresponding execution time (exec time) in seconds.

\input{Evaluation/SC20-files/lorenz-table}

We perform analysis for 20, 40, and
70 iterations. The second state variable, $y$, shows more worst-case variation.


==> Evaluation/TACO25-files/lorenz_table.tex <==
\begingroup
\small
\begin{table}[ht]
\centering
%\makebox[0pt][c]{\parbox{0.8\textwidth}{%
%\begin{minipage}[b]{0.5\hsize}
\begin{tabular}{ccccccc}
\toprule
\multirow{3}{*}{Lorenz} & \multicolumn{6}{c}{Window of Abstraction depth : (mindepth, maxdepth)} \\
\cmidrule(lr){2-7}
& \multicolumn{2}{c}{(10,20)} & \multicolumn{2}{c}{(15,25)} & \multicolumn{2}{c}{(20,40)} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
				 & err 		& \shortstack[1]{Exec \\Time}			 & err		& \shortstack[1]{Exec \\Time} 			& err 		& \shortstack[1]{Exec \\Time}  \\
lorenz20: x	 & \tb{5.69e-15} & \multirow{3}{*}{\tb{14s}}	 & \tb{5.88e-15} & \multirow{3}{*}{\tb{535s}} 	& \tb{5.64e-15}  & \multirow{3}{*}{\tb{545s}}  \\
lorenz20: y	 & \tb{1.25e-14}	&  		 				 & \tb{1.25e-14} &   		 				& \tb{1.24e-14}	& 	\\
lorenz20: z	 & \tb{4.75e-15}	&  		 				 & \tb{4.82e-15} &   		 				& \tb{4.72e-15}	& 	\\
\cmidrule(lr){2-7}
lorenz40: x	 & \tb{3.78e-14} & \multirow{3}{*}{29s}	 & \tb{3.91e-14}	& \multirow{3}{*}{1131s}	& \tb{3.75e-14}	& \multirow{3}{*}{1192s}	\\
lorenz40: y	 & \tb{9.11e-14} &     		 			 & \tb{9.33e-14}	&    		 				& \tb{9.02e-14}	& 	\\
lorenz40: z	 & \tb{7.08e-14} &     		 			 & \tb{7.09e-14}	&    		 				& \tb{6.95e-14}	& 	\\
\cmidrule(lr){2-7}
lorenz70: x	 & \tb{3.02e-13} & \multirow{3}{*}{\tb{50s}}	 & \tb{2.45e-13}	& \multirow{3}{*}{\tb{2088s}}	& \tb{2.45e-13}	& \multirow{3}{*}{\tb{2150s}}	\\
lorenz70: y	 & \tb{1.06e-12} &     		 			 & \tb{7.93e-13}	&    		 				& \tb{7.93e-13}	& 	\\
lorenz70: z	 & \tb{1.05e-12} &     		 			 & \tb{8.14e-13}	&    		 				& \tb{8.14e-13}	& 	\\
\end{tabular}
\caption{Error bounds for the three state variables in the Lorenz equation}
\label{tab:lorenz-table}
%\end{minipage}
%}
%}
\end{table}
\endgroup


==> Evaluation/TACO25-files/results_table1.tex <==

%\begingroup
%	\begin{table*}[ht]
%	\centering
%	\begin{threeparttable}[t]
%	%\setlength\tabcolsep{1.8pt}
%	\begin{tabular}{cccccccccc}
%	  \toprule
%	  %\multirow{3}{*}{Benchmarks} & \multicolumn{6}{c}{Absolute Error Bound} & \multicolumn{2}{c}{\multirow{2}{*}{Instability}} & \multirow{3}{*}{Profiling Err Expr} & \multirow{3}{*}{Shdw profiling} \\
%	  \multirow{3}{*}{Benchmarks} & \multicolumn{4}{c}{Worst case absolute error estimation} & \multicolumn{2}{c}{\multirow{2}{*}{\shortstack{Instability\\Jump}}} &  \multicolumn{2}{c}{\multirow{3}{*}{\shortstack[1]{Empirical \\{Profiling}}}}\\
%	  \cmidrule(lr){2-5} 
%	  &      \multicolumn{2}{c}{Opt} & \multicolumn{2}{c}{POpt} & & & &  \\
%	  \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10}
%	  &      {FP Err} & {ExecTime} & {FP Err} & {ExecTime} & {Opt} & {POpt} & {\shortstack[1]{Prof \\{Error Expr}}} & {\shortstack[1]{Shadow \\{profiling}}} & {\shortstack[1]{Instability \\{jump}}}\\
%	\midrule
%	% BM : 			1-err 	  & 1-exec  & 2-err      & 2-exec & 3-err     & 3-exec  & inst1-err  & inst2-err  & stat  &  shadow    
%	Barycentric\tnote{a}  	&  1.04e-15  & 39s     & 1.04e-15   & 38s    &  7.81   &  7.81   & 8.24e-16   &  4.6e-16   & 0.93 \\
%	SymSchur\tnote{a}		&  4.13e-16  & 5.5s    & 4.02e-16   & 44s    &  0.42   &  0.08   & 8.56e-17   &  2.3e-17   & 1.48e-08 \\
%	DistSinusoid\tnote{a}   &  {\bf inf} & --      & 7.17e-06   & 23.4   &  {\bf inf} & 3.17 & 2.56e-16   &  2.18e-15  & 4.8e-04 \\
%	Interpolator\tnote{c}	&  7.49e-14  & 1.34s   & 1.47e-14   & 0.58s  &  225    & 33.25   & 1.14e-14   &  5.32e-15  & 11.25 \\
%	Nonlin-Interpol			&  2.24e-14  & 0.4s    & 4.44e-16   & 1.12s  &  101    & 2.93    & 2.77e-16   &  3.9e-16   & 2.9 \\
%	EnclosingSp\tnote{a}  	&  4.41e-15  & 1.67s   & 4.41e-15   & 7.31s  &  12.63  & 4.19    & 1.89e-15   &  5.10e-16  & 3.96e-07 \\
%	cubicspline\tnote{c}	&  8.88e-15  & 1.6s    & 4.16e-16   & 1.32s  &  27     & 16      & 1.94e-16   &  2.7e-17   & 0.25 \\
%	linearfit               &  3.07e-16  & 1.02s   & 3.07e-16   & 1.04s  &  1.08   & 0.318   & 7.5e-17    & 2.58e-16   & 0.13 \\
%	jetApprox\tnote{c}		&  7.45e-15  & 3.45s   & 7.04e-15   & 3.16s  &  15.13  & 5.79    & 1.90e-15   & 1.64e-15   & 0.20 \\
%	SqDistPtSeg\tnote{a}	&  6.81e-13  & 7.5s    & 5.60e-13   & 42.16s &  317.58 & 150.63  & 5.9e-14    &  7.13e-14  & 7.14 \\
%	Squareroot\tnote{b}		&  1.77e-15  & 1.28s   & 1.77e-15   & 0.18s  &  2.68   &  2.68   & 6.10e-16   &  3.06e-17  & -- \\
%	Styblinski\tnote{c}		&  4.09e-14  & 2.01s   & 2.02e-14   & 1.31s  &  51.62  &  0.01   & 7.25e-15   &  3.30e-16  & 3.21e-07 \\
%	Test2\tnote{a}			&  7.90e-14  & 2.34s   & 7.65e-14   & 15s    &  101.9  &  3.02   & 2.43-14    &  2.07e-14  & 0.69 \\
%	ClosestPoint\tnote{a} 	&  9.98e-16  & 6.3s    & 9.15e-16   & 24s    &  4.89   &  4.1    & 5.56e-16   &  5.15e-16  & 2.6e-07 \\
%	SpherePt\tnote{a}   	&  6.43e-15  & 66s     & 6.16e-e15  & 255    &  0.87   &  0.82  & 1.71e-15    &  1.87e-16  & 7.14 \\
%	lead-lag\tnote{b}		&  2.49e-16  & 6.98s   & 2.49e-16   & 12.5s  &  0.04   &  0.04   & 8.23e-17   &  3,21e-18  & -- \\
%	EigenSphere\tnote{a}  	&  1.67e-15  & 480s    & 1.67e-15   & 540s   &  2.16   &  2.16   & 6.09e-16   &  4.4e-16   & 1.37e-07 \\
%	Jacobi\tnote{a}			&  4.82e-13  & 22s     & 4.09e-13   & 151s   &  81.33  &  55.5   & 5.69e-14   &  2.96e-14  & -- \\
%	Mol-Dyn\tnote{a}		&  2.94e-15  & 138s    & 2.94e-15   & 137s   &  2.11   &  2.11   & 1.39e-15   &  1.22e-15  & -- \\
%	Gram-Schmidt\tnote{b}	&  2.42e-16  & 99s     & 2.42e-16   & 226s   &  0.0284 & 0.0284  &  3.97e-17  &  3.88e-17  & 8.37e-04 \\
%	Ray Tracing\tnote{a}	&  4.70e-14  & 331s    & 4.65e-14   & 317s   &  87.7   &  0.129  &  1.42e-14  &  1.59e-16  & 2.90e-08 \\
%	ExtremePoint\tnote{a}	&  1.69e-14  & 30s     & 1.69e-14   & 33s    &  115.5  &  115.5  &  1.68e-14  &  1.0e-19   & 4.52e-06 \\  
%	SmartRoot\tnote{b}		&  {\bf inf} & --      & 2.44e-15   & 0.89s  &  {\bf inf}   &  0.526  & 3.90e-16   &  0    & 1.26e-07 \\
%	Poisson\tnote{a}		&  1.0e-17   & 120s    & 1.0e-18    & 121s   &  0.97   &  0.97   & 3.7e-18    &  2.33e-19  & -- \\
%	\end{tabular}
%	\begin{tablenotes}
%		\item[a] New benchmarks introduced with \seesaw for conditional codes
%		\item[b] Benchmarks ported from FPBench
%		\item[c] Benchmarks ported from PRECiSA
%	\end{tablenotes}
%	\caption{\label{tab:seesaw-solver-compare} \seesaw evaluation for worst case error bounds and instability reporting. }
%	\end{threeparttable}
%	\end{table*}
%\endgroup

\begingroup
	\begin{table*}[ht]
	\centering
	\begin{threeparttable}[t]
	%\setlength\tabcolsep{1.8pt}
	\begin{tabular}{crrrrrrrrr}
	  \toprule
	  %\multirow{3}{*}{Benchmarks} & \multicolumn{6}{c}{Absolute Error Bound} & \multicolumn{2}{c}{\multirow{2}{*}{Instability}} & \multirow{3}{*}{Profiling Err Expr} & \multirow{3}{*}{Shdw profiling} \\
	  \multirow{3}{*}{Benchmarks} & \multicolumn{4}{c}{Worst case absolute error estimation} & \multicolumn{2}{c}{\multirow{2}{*}{\shortstack{Instability\\Jump}}} &  \multicolumn{2}{c}{\multirow{3}{*}{\shortstack[1]{Empirical \\{Profiling}}}}\\
	  \cmidrule(lr){2-5} 
	  &      \multicolumn{2}{c}{Optimizer} & \multicolumn{2}{c}{Preconditioned Optimizer} & & & &  \\
	  \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-10}
	  &      {Error} & {ExecTime} & {Error} & {ExecTime} & {Optimizer} & {\shortstack[1]{Preconditioned \\{Optimizer}}} & {\shortstack[1]{Prof \\{Error Expr}}} & {\shortstack[1]{Shadow \\{profiling}}} & {\shortstack[1]{Instability \\{jump}}}\\
	\midrule
	% BM : 			1-err 	  & 1-exec  & 2-err      & 2-exec & 3-err     & 3-exec  & inst1-err  & inst2-err  & stat  &  shadow    
	Barycentric\tnote{a}  	&  1.04e-15  & 39.00s   & 1.04e-15   & 38.00s   &  7.81   	& 7.81    & 8.24e-16   &  4.6e-16   & 0.93 \\
	SymSchur\tnote{a}	&  4.13e-16  & 5.50s    & 4.02e-16   & 44.00s   &  0.42   	& 0.02    & 8.56e-17   &  2.3e-17   & 1.48e-08 \\
	DistSinusoid\tnote{a}   &  {\bf inf} & --       & 7.17e-06   & 23.40s   &  {\bf inf} 	& 3.17    & 2.56e-16   &  2.18e-15  & 0.05 \\
	Interpolator\tnote{c}	&  7.49e-14  & 1.34s    & 1.47e-14   & 0.58s  	&  225.00    	& 33.25   & 1.14e-14   &  5.32e-15  & 11.25 \\
	Nonlin-Interpol		&  2.24e-14  & 0.40s    & 4.44e-16   & 1.12s  	&  101.00    	& 2.93    & 2.77e-16   &  3.9e-16   & 2.9 \\
	EnclosingSp\tnote{a}  	&  4.41e-15  & 1.67s    & 4.41e-15   & 7.31s  	&  12.63  	& 4.19    & 1.89e-15   &  5.10e-16  & 4.74e-07 \\
	cubicspline\tnote{c}	&  8.88e-15  & 1.60s    & 4.16e-16   & 1.32s  	&  27.00     	&  0.25   & 1.94e-16   &  2.7e-17   & 0.25 \\
	linearfit               &  3.07e-16  & 1.02s    & 3.07e-16   & 1.04s  	&  1.08   	& 0.318   & 7.5e-17    &  2.58e-16  & 0.13 \\
	jetApprox\tnote{c}	&  7.45e-15  & 3.45s    & 7.04e-15   & 3.16s  	&  15.13  	& 5.79    & 1.90e-15   &  1.64e-15  & 0.20 \\
	SqDistPtSeg\tnote{a}	&  6.81e-13  & 7.50s    & 5.60e-13   & 42.16s 	&  317.58 	& 150.63  & 5.9e-14    &  7.13e-14  & 7.14 \\
	Squareroot\tnote{b}	&  1.77e-15  & 1.28s    & 1.77e-15   & 0.18s  	&  2.68   	&  2.68   & 6.10e-16   &  3.06e-17  & -- \\
	Styblinski\tnote{c}	&  4.09e-14  & 2.01s    & 2.02e-14   & 1.31s  	&  51.62  	&  0.01   & 7.25e-15   &  3.30e-16  & 3.21e-07 \\
	Test2\tnote{a}		&  7.90e-14  & 2.34s    & 7.65e-14   & 15.00s   &  101.90  	&  3.02   & 2.43-14    &  2.07e-14  & 0.69 \\
	ClosestPoint\tnote{a} 	&  9.98e-16  & 6.30s    & 9.15e-16   & 24.00s   &  4.59   	&  1.45   & 5.56e-16   &  5.15e-16  & 2.6e-07 \\
	SpherePt\tnote{a}   	&  6.43e-15  & 66.00s   & 6.16e-e15  & 255.00s  &  0.87   	&  0.82   & 1.71e-15   &  1.87e-16  & 1.02e-06 \\
	lead-lag\tnote{b}	&  2.49e-16  & 6.98s    & 2.49e-16   & 12.50s  	&  0.04   	&  0.14   & 8.23e-17   &  3,21e-18  & 1.51e-04 \\
	EigenSphere\tnote{a}  	&  1.67e-15  & 480.00s  & 1.67e-15   & 540.00s 	&  2.16   	&  2.16   & 6.09e-16   &  4.4e-16   & 1.37e-07 \\
	Jacobi\tnote{a}		&  4.82e-13  & 22.00s   & 4.09e-13   & 151.00s 	&  81.33  	& 55.50   & 5.69e-14   &  2.96e-14  & -- \\
	Mol-Dyn\tnote{a}	&  2.94e-15  & 138.00s  & 2.94e-15   & 137.00s 	&  2.11   	&  2.11   & 1.39e-15   &  1.22e-15  & 5.67e-06 \\
	Gram-Schmidt\tnote{b}	&  2.42e-16  & 99.00s   & 2.42e-16   & 226.00s 	&  0.02 	& 0.02    & 3.97e-17   &  3.88e-17  & 8.37e-04 \\
	Ray Tracing\tnote{a}	&  4.70e-14  & 331.00s  & 4.65e-14   & 317.00s 	&  87.70   	&  0.129  &  1.42e-14  &  1.59e-16  & 2.90e-08 \\
	ExtremePoint\tnote{a}	&  1.69e-14  & 30.00s   & 1.69e-14   & 33.00s  	&  115.50  	& 115.50  &  1.68e-14  &  1.0e-19   & 4.52e-06 \\  
	SmartRoot\tnote{b}	&  {\bf inf} & --       & 2.44e-15   & 0.89s   	&  {\bf inf}   	&  0.52   & 3.90e-16   &  0    	    & 1.26e-07 \\
	Poisson\tnote{a}	&  1.0e-17   & 120.00s  & 1.0e-18    & 121.00s 	&  0.97   	&  0.97   & 3.7e-18    &  2.33e-19  & -- \\
	\end{tabular}
	\begin{tablenotes}
		\item[a] New benchmarks introduced with \seesaw for conditional codes
		\item[b] Benchmarks ported from FPBench
		\item[c] Benchmarks ported from PRECiSA
	\end{tablenotes}
	\caption{\label{tab:seesaw-solver-compare} \seesaw evaluation for worst case error bounds and instability reporting. }
	\end{threeparttable}
	\end{table*}
\endgroup


==> Introduction/TACO25-contributions.tex <==
Our key contributions are as follows:
\begin{itemize}
    \item Extending symbolic error taylor forms with type-cast rounding.
    \item Extending benchmark suite with mixed-precision and uniform single-precision benchmarks. 
\end{itemize}

==> Mixed_Precision_Extension/TACO25-files/extending_error_taylor_form.tex <==
\noindent{\bf {Extending Error Taylor Forms}:\/}

We can now extend the rounding model specified in Eq~\ref{eq:floating-point-operation} using the additional type-cast rounding:

\begin{equation} \label{mixed-precision-floating-point-operation}
    \begin{split}
        \circ(\Tilde{x} \diamond \Tilde{y}) &= (\Tilde{x} \diamond \Tilde{y})(1 + \delta)(1+\Delta) \\
                                            &= (\Tilde{x} \diamond \Tilde{y}) + (\Tilde{x} \diamond \Tilde{y})\delta + (\Tilde{x} \diamond \Tilde{y})\Delta + (\Tilde{x} \diamond \Tilde{y})\delta\Delta, |\delta|,|\Delta| \leq \mathbf{u}
    \end{split}                          
\end{equation}

We thus introduce the additional error term $\mathcal{T}(\mathscr{S}) = (\Tilde{x} \diamond \Tilde{y})\Delta$ representing the amount of round-off error due to type-casting. Note that we ignore the term $(\Tilde{x} \diamond \Tilde{y})\delta\Delta$ since we ignore all higher-order error.

Considering the straight-line program in \S\ref{subsec:taylor_expansion} with n floating-point sub-expressions, we now have their finite precision counter-parts including type-cast rounding errors as follows,

\begin{align*}
	\tilde{\mathscr{S}_i} 
	&= \tilde{\dot{\mathscr{S}_i}}(\tilde{x}_1, \dotsc, \tilde{x}_m, \mathscr{S}_1, \dotsc, \mathscr{S}_{i-1}) \\
	&= \tilde{\dot{\mathscr{S}_i}}(x_1+\mathcal{E}^{lr}_{x_1}+\mathcal{T}_{x_1},\dots,x_m+\mathcal{E}^{lr}_{x_m}+\mathcal{T}_{x_m}, \mathscr{S}_1 + \mathcal{E}^{lr}_{\mathscr{S}_1} + \mathcal{T}_{\mathscr{S}_1}, \dotsc, \mathscr{S}_{i-1} + \mathcal{E}^{lr}_{\mathscr{S}_{i-1}} + \mathcal{T}_{\mathscr{S}_{i-1}}) \\
    &= \dot{\mathscr{S}_i}(x_1+\mathcal{E}^{lr}_{x_1}+\mathcal{T}_{x_1},\dots,x_m+\mathcal{E}^{lr}_{x_m}+\mathcal{T}_{x_m}, \mathscr{S}_1 + \mathcal{E}^{lr}_{\mathscr{S}_1} + \mathcal{T}_{\mathscr{S}_1}, \dotsc, \mathscr{S}_{i-1} + \mathcal{E}^{lr}_{\mathscr{S}_{i-1}} + \mathcal{T}_{\mathscr{S}_{i-1}})( 1 + \delta_i)(1+\Delta_i);
	\quad |\delta_i| \leq \bf{u}
\end{align*}
We can now express the error $\mathcal{E}^{tr}_{\mathscr{E}_{n}}$ of the program output as
\begingroup
\small
\begin{equation*}
\begin{split}
	\mathcal{E}^{tr}_{\mathscr{E}_{n}}
	&= \dot{\mathscr{E}_n}(x_1+\mathcal{E}^{lr}_{x_1}+\mathcal{T}_{x_1},\dots,x_m+\mathcal{E}^{lr}_{x_m}+\mathcal{T}_{x_m}, \mathscr{S}_1 + \mathcal{E}^{lr}_{\mathscr{S}_1} + \mathcal{T}_{\mathscr{S}_1}, \dotsc, \mathscr{S}_{i-1} + \mathcal{E}^{lr}_{\mathscr{S}_{n-1}} + \mathcal{T}_{\mathscr{S}_{n-1}})( 1 + \delta_n)(1+\Delta_n) - \mathscr{E}_n;\quad |\delta_n| \leq \bf{u}
\end{split}
\end{equation*}
\endgroup

Performing a Taylor expansion about zero for all error values, we get:
\begingroup
\small
\begin{equation}
\label{eq:mixed-precision-taylor-expansion}
   \mathcal{E}^{tr}_{\mathscr{E}_{n}} = \mathscr{E}_n\delta_n
            + \sum_{j=1}^{n-1} \dfrac{\partial \mathscr{E}_n}{\partial \mathscr{S}_j}(\mathcal{E}^{lr}_{\mathscr{S}_j} + \mathcal{T}_{\mathscr{S}_j})
            + \sum_{j=1}^{m} \dfrac{\partial \mathscr{E}_n}{\partial x_j}(\mathcal{E}^{lr}_{x_j} + \mathcal{T}_{x_j})
            + O({\bf u}^2)
\end{equation}
\endgroup

==> Mixed_Precision_Extension/TACO25-files/type_cast_rounding.tex <==
% \noindent{\bf {Type Cast Rounding}:\/}
\subsection{Type-Cast Rounding}

Let $A^\mathscr{E}$ (denoted as A when $A^\mathscr{E}$ is clear) be a mapping from the post-order numbering of operators in $\mathscr{E}$ to the set of machine epsilons $(\epsilon_{64}, \epsilon_{32}, \epsilon_{16})$. For instance, an expression $\mathscr{E}=x+y$ with x set to single-precision, y set to double precision and the + operator yielding a single-precision output, will have a mapping $A^\mathscr{E} = {(0, \epsilon_{32}), (1, \epsilon_{64}), (2, \epsilon_{32})}$.

When an operator yields an output of a certain precision, we assume its inputs to be set to the same precision. The operator thus forms the context for its inputs. In our example, a type-cast operation is needed to round-down the input y from double-precision to single-precision. The `+` operator thus forms the context for its inputs x and y in determining type-cast operations. These type-cast operations introduce $\emph{additional}$ round-off errors. Note that since we do not know the context for the `+' operator, we assume the rounding-error due to type-cast to be 0.

==> illustrative_example/illustrative_example.tex <==
\section{Illustrative Example}
\begin{itemize}
    \item Building Computational Graph
    \item Generating and Accumulating Error
    \begin{itemize}
        \item Local Error propagation
        \item Type Cast error generation
        \item Predicate Weakening
        \item Error Accumulation
    \end{itemize}
    \item Constraint generation
    \item Global Optimization
    \item Instability analysis
\end{itemize}



